MilliSonic: Pushing the Limits of Acoustic Motion Tracking

Recent years have seen interest in device tracking and localization using acoustic signals. State-of-the-art acoustic motion tracking systems however do not achieve millimeter accuracy and require large separation between microphones and speakers, and as a result, do not meet the requirements for many VR/AR applications. Further, tracking multiple concurrent acoustic transmissions from VR devices today requires sacrificing accuracy or frame rate. We present MilliSonic, a novel system that pushes the limits of acoustic based motion tracking. Our core contribution is a novel localization algorithm that can provably achieve sub-millimeter 1D tracking accuracy in the presence of multipath, while using only a single beacon with a small 4-microphone array.Further, MilliSonic enables concurrent tracking of up to four smartphones without reducing frame rate or accuracy. Our evaluation shows that MilliSonic achieves 0.7mm median 1D accuracy and a 2.6mm median 3D accuracy for smartphones, which is 5x more accurate than state-of-the-art systems. MilliSonic enables two previously infeasible interaction applications: a) 3D tracking of VR headsets using the smartphone as a beacon and b) fine-grained 3D tracking for the Google Cardboard VR system using a small microphone array.

==> sections/abstract_0.tex <==
\begin{abstract}

Recent years have seen various optical motion tracking techniques for VR/AR systems. However, they require dedicated base stations and controllers. Acoustic solution appeard to be an attractive alternative because of the ubiquity of speakers and microphones. However, existing solutions stagnate at around 1cm accuracy and require a large speaker/microphone separation, both not suitable for AR/VR applications.

%Recent years have seen interest in device xXXtracking and localization using acoustic signals from.  XXX




    We present \name, a high-precision acoustic motion tracking system.
    The core of \name is a novel localization algorithm leveraging the phase of the demodulated FMCW signals. We additionally address the phase ambiguity and synchronization issue to achieve reliable continuous tracking. 
    Without sacrificing latency or refresh rate, \name achieves a sub-mm level 1D distance accuracy and a 2.6mm median 3D tracking accuracy for smartphones using a $15cm\times 15cm$ 4-microphone array, approximately 5x more accurate than the state-of-the-art.
    
    \name enables two previously unfeasible interaction methods between smartphones/smartwatches and VR/AR headsets: a) tracking headsets without beacons by putting your smartphone on the table, and use your smart watch to track arm motion; b) tracking the position of smartphone-based VR headsets using a cheap and small microphone array. 
    Our extensive evaluation and user study validates the high accuracy and interactivity of \name.
\end{abstract}

==> sections/concurrent_0.tex <==
\section{Concurrent Tracking}

Concurrent tracking is an important feature because there would exist multiple devices to be tracked at the same time.
Traditionally, wireless protocols support multiple transmissions using time-division multiplexing (TDM), or frequency-division multiplexing (FDM). In short, each transmission is only allowed to use a portion of time slices or frequency bands, which is determined by a scheduling protocol. 

However, both TDM and FDM are not suitable for concurrent motion tracking. Specifically, by using TDM, each transmission would have a lower refresh rate inverse-proportional to the number of transmissions; by using FDM, the bandwidth for each transmission is reduced, which affects the accuracy.

Keep these in mind, we utilize two essential properties of MilliSonic to support concurrent tracking without sacrificing accuracy nor agility.

\subsubsection{One-way transmission}
The whole MilliSonic algorithm described above is one-way, which means signals are only propagated from the transmitter to the receiver. 
Because of this, MilliSonic can support unlimited number of receivers to be tracked by one single transmitter.

\subsubsection{Orthogonality of FMCW signals}
Different from optical signals, acoustic signals are omni-directional by nature. Concurrent transmissions from multiple speakers share a same transmission medium. 
By definition from Eq.~\ref{eq:fmcwdemod}, for two received FMCW paths with a time-of-arrival difference of $\delta t$, their dot product has a bound of $[-\frac{T}{B\pi\delta t}, \frac{T}{B\pi\delta t}]$. This indicates when two paths have a long time-of-arrival difference, they are nearly orthogonal to each other.  

Utilizing this fact, we can support concurrent transmissions from multiple speakers by introducing a \textit{virtual} time-of-arrival offset. 

At the beginning, $N$ transmitters transmit FMCW chirps one by one to the receiver. The receiver know their time-of-arrivals using our algorithm, denoted by $t_d^{(i)}$ for the $i$th transmitter. 
The receiver sends back $\frac{iT}{2N}-t_d^{(i)}$ to each transmitter $i$, which is the virtual offset for transmitter $i$. The receiver $i$ then intentionally delays its transmission by its virtual offset. In this way, all transmitters can start transmissions concurrently.  
 
On the receiver side, there exist $N$ separate peaks evenly distributed on the frequency domain, which corresponds to $N$ evenly distributed time-of-arrivals in $[T/2N, T/2]$, where the $i$th time-of-arrival is from the $i$th transmitter. 
The receiver can regard transmissions from other transmitters as multipath. Because of the orthogonality, they are filtered out by the band-pass filter at the first step. It can then track the phase of each of them using five different band-pass filters without losing accuracy nor agility. 
After calculating the time-of-arrival of the signal from each transmitter, it subtracts the virtual offset from it and obtain the final result. 

Because of motion, if multiple peaks merge together the receiver would not track any of them, so essentially this trades off the working range of each transmitter. 
However, this limitation can be mitigated: the receiver can send back a new set of delays periodically to assign a new evenly distributed time-of-arrival offset.

==> sections/design-3.tex <==
\section{\name\ Design}
We first present background on existing FMCW tracking systems and show why they have a limited accuracy for acoustic tracking. We then present our algorithm that uses the FMCW phase to achieve sub-mm 1D tracking. We then describe how to perform 3D tracking using the 1D locations using multiple microphones. Finally, we address various practical issues. % including synchronization, phase ambiguity as well as  failure detection and recovery.

%To avoid catastrophic errors due to occlusions or noises, we also design a classification method to reset the states when failure happens.

%

% The hardware setup is shown in Fig.~\ref{fig:setup}. A \textit{gadget receiver} consists of one speaker and four microphones sitting on four corners in a $15cm\time 10cm$ rectangle. A \textit{transmitter}, which can be another gadget receiver, a smartphone, or a customized device, requires one speaker and one microphone embedded.

% We first review two traditional motion tracking methods.

\subsection{FMCW Background}

Acoustic tracking is traditionally achieved by computing  the time-of-arrival of the transmitted signals at the microphones.  At its simplest, the transmitted signal is a sine wave, $x(t)=exp(-j2\pi ft)$ where $f$ is the wave frequency. A microphone at a distance of $d$ at the transmitter, has a time-of-arrival of \red{$d = t_d * c$} where $c$ is the speed of sound. The received signal at this distance can now be written as, $y(t) = exp(-j2\pi t(t-t_d)$. Dividing by $x(t)$, we get $\hat{y}(t)=\exp(j2\pi ft_d)$. Thus, the phase of the received signal can be used to compute the time-of-arrival, $t_d$. In practice, however, multipath significantly distorts the received phase limiting accuracy. 

To combat multipath, prior work~\cite{mao2016cat, nandakumar2015contactless} uses  Frequency Modulated Continuous Wave (FMCW) chirps where as shown in Fig.~\ref{fig:fmcw} the frequency of the signal changes linearly with time. FMCW has good autocorrelation properties that allow the receiver to \red{differentiate} between multiple paths that each have a different time-of-arrival. \red{Compared with OFDM\cite{fingerio} or other CAZAC waveforms \cite{cazac}, FMCW has high spectral efficiency and ease of demodulate. }

Mathematically, the FMCW signal in Fig.~\ref{fig:fmcw} is,
 $$x(t)=exp(-j2\pi (f_0+\frac{B}{2T}t)t) = 
 exp(-j2\pi (f_0t+\frac{B}{2T} t^2))$$ where $f_0$, $B$ and $T$ are the initial frequency, bandwidth and duration of the FMCW chirp respectively. In the presence of multipath, the received signal can be written as, $$y(t)=\sum_{i=1}^M A_iexp(-j2\pi(f_0(t-t_i)+\frac{B}{2T} (t^2+t_i^2-2tt_i)))$$ where $A_i$ and $t_i=\frac{d_i(t)}{c}$ are the attenuation and time-of-flight of the $i$th path at time $t$. Dividing this by $x(t)$ we get,
\begin{align}
\hat{y}(t)&=\sum_{i=1}^M A_iexp(-j2\pi (\frac{B}{T}t_it+f_0t_i-\frac{B}{2T}t_i^2)) \label{eq:fmcwdemod}
\end{align}
The above equation shows that multipath with different times-of-arrival fall into different frequencies. The receiver uses \red{Discrete Fourier Transform (DFT)} to find the first peak frequency bin, $f_{peak}$, that corresponds to the line-of-sight path to the transmitter. It then computes the distance to the receiver as, $d(t)=\frac{cf_{peak}}{B}$.


While this conventional FMCW processing is effective in disambiguating multiple paths that is separated by large distances, it has a limited accuracy when the multiple paths are close to each other. Specifically, the minimum distance resolution for FMCW is in the order of $\frac{c}{B}$ when the separation between frequencies is 1~Hz. Given that smartphones have a limited inaudible bandwidth of {7~kHz} between {17-24~kHz}, prior work cannot distinguish between paths that are close to the direct line-of-sight path and hence have a limited accuracy~\cite{mao2016cat, peng2007beepbeep}. Further, since FFT operations are performed over a whole chirp duration, it limits the frame rate of the system to $\frac{1}{T}$, where $T$ is the FMCW chirp duration.


\begin{figure}
\includegraphics[width=0.3\textwidth]{images/fmcwsimple.pdf}
\vskip -0.15in
\caption{FMCW signal structure.}
\vskip -0.15in
\label{fig:fmcw}
\end{figure}

\subsection{Sub-mm 1D tracking using FMCW phase}

Our intuition is that the phase of the FMCW signals can also be used to compute distance. Thus, instead of  using the first peak frequency of the FMCW signal in the frequency domain to estimate the time-of-arrival, our algorithms has two key steps: 1) we apply a dynamic narrow band-pass filter in the time-domain to filter out most multipath that has a distant time-of-arrival from the direct path. This leaves us only a small portion of residual indirect paths around the direct path. 2) We  then extract the distance information from the instantaneous phase of the FMCW signals. We show that this algorithm has 10x higher accuracy than prior FMCW systems that track the peak frequency to estimate distance.

{\it 1) Adaptive band-pass filter to remove distant multipath.}  For the first FMCW chirp, we extract the first peak of the demodulated signal in the frequency domain using an DFT similar to prior designs from Eq.~\ref{eq:fmcwdemod}. We then apply a \red{Finite Impulse Response (FIR)} filter that only leaves a narrow range of frequency bands around the peak. The delay of the FIR filter need to be carefully chosen: if it is too small, it cannot filter most indirect paths and also leaves a lot of noise; if it is too large, it will introduce more latency and require more gap between consequent chirps to prevent interference. This results in reducing the maximum supported acceleration. In our algorithm, we adaptively set the delay of the FIR filter from the SNR of the acoustic signals. Specifically, when $SNR>10dB$, we use a 15ms delay; otherwise, we double the delay to $30ms$.

For subsequent FMCW chirps we no longer use the DFT to extract the peak frequency. Instead, for the $i+1$th FMCW chirp, we infer the new peak from the distance and speed estimated at the end of the $i$th chirp. We then apply the FIR filter around this new peak. Given the distance $d^{(i)}_{end}$ and speed $v^{(i)}_{end}$ estimated from the end of the $i$th chirp, we can infer the distance of the beginning of the current chirp  $\hat{d}^{(i+1)}_{start}=d^{(i)}_{end}+v^{(i)}_{end}\delta T$ where $\delta T$ is the gap between two chirps. We do this for two key reasons: a) our distance estimates are far more accurate than the peak of the DFT result; and b) unlike a DFT that is performed over a whole FMCW chirp, we do not require receiving a full FMCW chirp before processing, thus reducing the frame rate. 

Finally, we note that Doppler effects can blur the peak in the frequency domain. To address this, we adaptively increase the width of the pass band in the FIR filter when the speed estimate at the end of the previous chirp exceeds a given threshold. In our algorithm, we set the pass band width to $1Hz$ when the speed does not exceed $1m/s$; otherwise, we set the pass band width to $2Hz$. 


{\it 2) Extracting distance from FMCW phase.} The above process eliminated all multipaths that have a much larger time-of-flight than the direct path. This leaves us with residual indirect paths around the direct path. \red{Empirically, when there is no occlusions, the sum of the residual indirect paths does always have a lower amplitude than the direct path.} 

We next describe how we extract the distance from the phase value. We also prove why this method has 10x better accuracy than prior FMCW tracking algorithms in the presence of multipath.

Specifically, to extract the distance from the phase value, we approximate the effect of residual multipath after filtering. From Eq.~\ref{eq:fmcwdemod}, we approximate the phase as,
\begin{equation}
\mathbf{\phi}(t) \approx -2\pi(\frac{B}{T}tt_d+f_0t_d-\frac{B}{2T}t_d^2)
\label{eq:phasequadratic}
\end{equation}
where $t_d$ is the time of arrival of the direct path. The approximation is assuming that we have already applied the dynamic filter to remove most multipath that has a much larger time-of-arrival distance than the direct path. We then approximate the residual indirect paths and noise to be 0. 

We solve \red{Eq.~\ref{eq:phasequadratic}} to get an instantaneous estimate of $t_d$ given the  instantaneous phase $\phi(t)$\footnote{There are two solutions to this quadratic equation; the other solution is out of the range of the FMCW chirp, $[0, T]$.}:

\begin{equation}
t_d(t, \phi(t)) \approx \frac{-2\pi(\frac{B}{T}t+f_0)+\sqrt{4\pi^2(\frac{B}{T}t+f_0)^2+4\pi\frac{B}{T}\phi(t)}}{-2\pi\frac{B}{T}} \label{eq:quadraticsolution}
\end{equation}

\begin{figure}
`\includegraphics[width=0.2\textwidth]{images/phaseerror.pdf}
\vskip -0.15in
\caption{Phase error when one indirect path (red vector) is combined with the direct path (blue vector).}
\vskip -0.15in
\label{fig:phaseerror}
\end{figure}

The distance $d(t, \phi(t))$ can then be computed as, $ct_d(t, \phi(t))$. The key observation we make in this paper is that the distance derived from the phase using Eq.~\ref{eq:quadraticsolution} is much more sensitive than the distance derived from the frequency peak in prior work. Specifically, we show the following.

\begin{lemma} Assume that the amplitude of the residual indirect paths after filters have a lower amplitude than the direct path. Now, given that $A_1$ and $A_2$ are the amplitude of the direct path and the total amplitude of the residual indirect paths, the phase error is upper bounded by $sin^{-1}(\frac{A_2}{A_1})$.
\end{lemma}
\begin{proof}
In Fig.~\ref{fig:phaseerror}, the complex representation of the direct path is represented by the blue vector while that of the sum of indirect paths is represented by the red vector. The sum of the two vectors is the resulting signal at the receiver which is represented by the green vector. The maximum phase error occurs when the red vector is perpendicular to the green vector and this corresponds to a phase error of $sin^{-1}(\frac{A_2}{A_1})$.
\end{proof}
\begin{lemma} Given the above phase error bound, the error in our distance estimate, $d(t)$ from Eq.~\ref{eq:quadraticsolution} is upper bounded by $\frac{sin^{-1}(A_2/A_1)c}{2\pi(f_0-B/2)}$, where $f_0$ and $B$ are the FMCW parameters. 
\end{lemma}
\begin{proof} See Appendix for the proof.
\end{proof}


\begin{figure}
\includegraphics[width=0.4\textwidth]{images/errcmp.eps}
\vskip -0.15in
\caption{Error comparison of FMCW peak vs. our method.}
\vskip -0.15in
\label{fig:errcompare}
\end{figure}


We compare this to the traditional peak estimation method for FMCW signals. We denote the time-of-arrival of the direct path as $t_1$ and its frequency in the demodulated FMCW signal as $\mathbf{f}_{t_1}$. An indirect path with a time-of-arrival of $t_2$ lies at frequency $\mathbf{f}_{t_2}$ in the demodulated signal. When $|\mathbf{f}_{t_1}-\mathbf{f}_{t_2}|<1$, 
the two peaks merge together in the frequency domain resulting in a single peak at approximately $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)$. Hence, the frequency error is $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)-\mathbf{f}_{t_1}$ which is equivalent to a distance error given by,  
$%\begin{equation*}
d_e^{(peak)}=(\frac{A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1}}{A_2+A_1}-\mathbf{f}_{t_1})\frac{c}{B} = \frac{\mathbf{f}_{t_2}-\mathbf{f}_{t_1}}{1+\frac{A_1}{A_2}} \frac{c}{B}
%\label{eq:disterr1}
$.%\end{equation*}

Fig.~\ref{fig:errcompare} shows that distance error as a function of $A_2/A_1$ and $|\mathbf{f}_{t_2}-\mathbf{f}_{t_1}|$ for both traditional peak estimation techniques as well as our method. The plots show that the distance errors using peak estimation is severely affected by the time-of-flight of the indirect paths. In contrast,  the distance error using our FMCW phase technique is around 10x lower.



\subsection{3D tracking from 1D locations}

The above FMCW phase technique allows us to achieve sub-mm resolution in estimating 1D distances. To achieve 3D tracking we use information from multiple microphones to perform triangulation.  We use multiple microphones instead of speakers to reduce the power consumption as well as to eliminate the complexity of multiplexing the multiple speakers. Since our 1D resolution is high we can also reduce the separation between the microphones  while achieving a good 3D accuracy. Specifically, we place four microphones at four corners of a rectangle.  We have two pairs of microphones in the vertical position and the other two pairs in the horizontal position. Thus, by computing the intersection of all the resulting 1D positions, we can compute the 3D location. 

We note that the accuracy of triangulation is dependent on the distance from the microphone array as well as the separation between the microphones. Specifically, as the distance from the microphone array increases, the resulting 3D accuracy become worse. Similarly, as the separation between microphones increase the 3D accuracy improves, which is why prior work uses a microphone separation of 90~cm~\cite{mao2016cat}. In our solution, since we already achieve sub-mm 1D resolution, we can reduce the separation between microphones to fit the form-factor of VR headset and still achieve good 3D tracking accuracies upto 2~m.  To improve the accuracy and reduce jitters at larger distances, we average the 3D distance measurements within each 10ms duration. Incorporating the 15ms latency of the band-pass filter, we get one distance value every 25ms or a frame rate of 40 frames per second. \red{Note that sensor fusion with IMU can further improve the frame rate which we leave for future work.}


%We however still need to address several important problems to achieve continuous high accuracy acoustic tracking. 

\subsection{Addressing practical issues}
We describe the practical issues in designing \name.







{\it 1) Phase ambiguity.} Any phase tracking algorithm has to address the problem of phase ambiguity. 
Specifically, we can only extract the phase modulo $2\pi$ from the demodulated chirp ($\hat{\phi}(t)=\mathbf{\phi}(t)\text{ mod }2\pi$).
This leads to two problems: a) how to detect any modulo $2\pi$ shifts during a single chirp; and b) how to estimate the initial $2N\pi$ phase offset, \textit{i.e.,} $\mathbf{\phi}(0)=2N\pi+\hat{\phi}(0)$ at the beginning of each chirp.

\red{Because of the band-pass filter, adjacent samples does not have a phase difference of more than $\pi$. The phase error caused by residual indirect paths is bounded to $(-\pi/2, \pi/2)$. Hence, multipath error does not cause a more than $\pi$ phase jump as well. As a result,} when the phase modulo $2\pi$ sees a sudden jump of more than $\pi$/$-\pi$ between adjacent time samples, $t$ and $t-\delta t$, we know there is a modulo $2\pi$ jump at that time, which we can correct by adding or subtracting $2\pi$ to the computed phase.

To compute the initial $2N\pi$ phase offset at the beginning of each chirp, we use the estimated distance and speed from the end of the previous chirp. Instantaneous speed is computed by performing least square linear regression (which is a linear algorithm in 1D domain) over the distance values in a 10~ms window to reduce the effects of noise and residual multipath. 


Specifically, for the $i+1$th received chirp, given the distance $d^{(i)}_{end}$ and speed $v^{(i)}_{end}$ estimated from the end of the $i$th chirp, we can infer the distance of the beginning of the current chirp  $\hat{d}^{(i+1)}_{start}=d^{(i)}_{end}+v^{(i)}_{end}\delta T$ where $\delta T$ is the gap between two chirps. 
We then find the $2N\pi$ offset in addition to the ambiguous initial phase $\hat{\phi}(0)$ that minimize the difference $|d^{(i+1)}(0, \hat{\phi}(0)+2N\pi)-\hat{d}^{(i+1)}_{start}|$. Note that this relaxes the constraints on speed imposed by prior work~\cite{mao2016cat} and instead has a constraint on acceleration. Specifically, prior work~\cite{mao2016cat} had a  constraint on the maximum speed of 1~m/s. In our algorithm, since each  $2\pi$ difference of the phase corresponds to around $2$~cm distance difference, any error smaller than $1$cm will not cause an erroneous $2N\pi$ estimate. The gap between two adjacent chirp is 5~ms and the delay of the band-pass filter is 15~ms.  Hence, as long as the acceleration does not exceed $\frac{1cm}{20ms \times 20ms}=25m/s^2$, our algorithm does not introduce erroneous phase offsets.
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.45\textwidth]{images/concurrent.pdf}
    \vskip -0.15in
    \caption{Supporting concurrent transmissions using virtual time-of-arrival offsets at each VR headset.}
    \vskip -0.25in
    \label{fig:prototype}
\end{figure}

{\it 2) Clock synchronization.} Clock differences exist in practice which we need to calibrate to achieve tracking. Specifically, we need to calibrate for the initial phase as well as any drift due to clock differences.  To achieve this, at the beginning of the session,  the user touches the smartphone speaker with a microphone at the receiver.  The receiver meanwhile starts recording the chirp for five seconds and runs the above tracking algorithm. Using this setup, we use autocorrelation to determine a starting time for the chirp at the receiver. Because in this setup, at zero distance, the signal has a high SNR, there is no motion and little indirect path, the estimate of the distance from the peak of the FFT result, denoted by $D$, is accurate.  As a result,  we can find the initial $2N\pi$ phase offset from $D$. Specifically, we find the best $2N\pi$  which minimizes the differences of the two measurements $|D-d(0, \hat{\phi}(0)+2N\pi)|$. Finally, to address the clock drift, the receiver detects a constant drift in {the distance measurement} within the five seconds which is linear to the clock difference. We then compensate the clock difference by removing this drift for the following measurements at the receiver side. 



{\it 3) Failure detection and recovery.} Our algorithms relies on continuous tracking. When tracking failure occurs, the subsequent measurements are also prone to errors.  In practice, failures occur due to  occlusions and  noise.  

While acoustic signal can penetrate some occlusions like fabrics, for other occlusions like wood and human limbs, refraction between different transmission mediums causes a dense multipath around the
direct path which is also greatly attenuated. Therefore, the above algorithm fails because it doesn't satisfy the premise that the direct path dominates the filtered demodulated signal. When such error happens during a chirp, it will cause fluctuations in phase. Thus, there would be multiple $2\pi$ phase tracking error during the chirp, leading to a larger than $2cm$ distance error at the end of the chirp. When the error happens between two chirps, it will lead to wrong $2N\pi$ estimate that causes larger than $~2cm$ error for the subsequent chirps. Similarly at longer ranges the signal attenuates which results in noisy phase measurements which can also lead to wrong $2N\pi$ estimates.


To detect these failures, we utilize the redundancy across the microphones. It is  unlikely that all the four microphone encounter the same extra phase error at the same time because of their different locations. Hence, if the measurements from some of the four microphones are outliers with at least $2cm$ measurement errors from the others, it indicates an error. 
When such a failure is detected, if the anomaly is only in one microphone, the receiver compensates the $2\pi$ offset until it is in the similar range of the other three microphones. If sustained failures occurs (which rarely happens), our algorithms fall back to the traditional peak estimation method for FMCW signals and notify the user.



\begin{figure}[t!]
    \centering
    \begin{subfigure}{0.178\textwidth}
    \includegraphics[width=1\textwidth]{images/minisonic.jpg}
    \caption{$6cm\times 5.35cm$}
    \end{subfigure}
    \hspace{2em}
    \begin{subfigure}{0.18\textwidth}
    \includegraphics[width=1\textwidth]{images/form15.jpg}
    \caption{$15cm\times 15cm$}
    \end{subfigure}
    \vskip -0.15in
    \caption{Prototypes of MilliSonic microphone arrays.}
    \vskip -0.15in
    \label{fig:minisonic}
\end{figure}


==> sections/design_0.tex <==
\section{Sub-mm level motion tracking}

\red{Applications: a) AR glasses - track smartphone as controller; b) smartphone as basestation - track AR glasses without vision; c) AR glasses - AR glasses co-localization in group play. }

Our key contribution to enable the above applications is a novel software pipeline to achieve sub-mm level motion tracking using acoustic signals that can be emitted and received by cheap microphone and speaker components or smartphones and smart watches. 
At a high level, our algorithm achieves sub-mm level tracking accuracy by solving the instantaneous phase of the signal meanwhile rejecting indirect multipaths. 
The speaker transmits an inaudible sound signal at frequency range of 17-23kHz. The microphones receive the acoustic signal samples which are passed through a series of low-complexity algorithms in real time. The precise 3D motion can be computed in a delay as short as 17.5ms.  

In the rest of this section, we first provide an overview of previous motion tracking methods. We then propose our algorithms to reduce the error by approximately 10x while supporting arbitrary motion speed and greatly reducing the delay time. We also design simple methods to address the synchronization problem which is a key problem in distributed systems. Finally, taking advantage of extremely accurate 1D measurements, 3D measurement can be computed accurately by using four microphones with a displacement of as small as $15cm\times 10cm$ which can be embedded in the AR glasses. 

The hardware setup is shown in Fig.~\ref{fig:setup}. A \textit{gadget receiver} consists of one speaker and four microphones sitting on four corners in a $15cm\time 10cm$ rectangle. A \textit{transmitter}, which can be another gadget receiver, a smartphone, or a customized device, requires one speaker and one microphone embedded.


\begin{figure}
\includegraphics[width=0.3\textwidth]{images/setup.png}
\caption{Hardware setup of \name.}
\label{fig:setup}
\end{figure}

We first review two traditional motion tracking methods.

\subsection{Phase Tracking}

The transmitter transmit a sine wave $x(t)=exp(-j2\pi ft)$. When there is no multipath, the receiver will receive a delayed signal $y(t)=exp(-j2\pi f(t-\frac{d(t)}{c}))$ where $d(t)$ is the distance between the pair at time $t$, and $c$ is the speed of sound.

The receiver can then downsample the signal by multiplying the carrier wave 
\begin{align}
\hat{y}(t)&=exp(-j2\pi f(t-\frac{d(t)}{c})+j2\pi ft) \nonumber\\
&=exp(j2\pi f\frac{d(t)}{c})
\label{eq:phasetracking}
\end{align}
We can then get the instantaneous phase of it for each $t$ to track the distance $d(t)$. 
Phase tracking is sensitive as a small as 1.6cm displacement would lead to a $2\pi$ phase change. It also introduces negligible delay which only depends on the band pass filter.

However, there are two major problems of this method. Firstly, there exist ambiguity in the phase, \textit{i.e.}, the phase we get from the signal $\phi(t)=(2\pi f\frac{d(t)}{c}) \text{mod} 2\pi$. Because of the modulus operation, we can only get the relative motion but not the absolute distance.
Secondly, when multipath exists, it will lead to severe interference to the combined phase. Single sine wave has no capability to separate multipath. Huge error can be introduced even with the existence of one indirect path. Previous works mitigate this problem by either using multiple frequencies \cite{LLAP}, or introducing sparsity constraint \cite{singleAPWifi}, but it either can only statistically reduce the error linearly to the limited number of frequencies, or requires huge computation of iterative approximate algorithms. 



\subsection{FMCW Tracking}

Another method is to use linear Frequency Modulated Continuous Wave (FMCW) signals (Fig~\ref{fig:fmcw}). Thanks to the good autocorrelation property of FMCW chirps, the receiver is able to differentiate different time-of-arrivals from a single received chirp. For linear FMCW signal, receiver can first demodulate by multiplying the same chirp in the time domain, pass through a low-pass filter, doing FFT and find the peak (Fig~\ref{fig:fmcw}). 

Despite most of multipaths can be separated out because of the property of FMCW signals, FMCW tracking has four major shortcomings. Firstly, it does not have a good sensitivity because the precision is limited by the sampling rate and FFT bins, which does not scale computationally. Secondly, indirect paths cannot be totally removed, as nearby paths with a distance separation of less than $O(\frac{c}{2B})$ would merge with the direct path and cause peak deviations. Third, Doppler effect caused by high speed motion can blur the FFT result and also introduces an additional bias to the peak estimate. Traditional solution is to use an upchirp followed by a downchirp which have opposite biases that can be canceled out, but it also doubles the processing delay.
Last but not the least, receiver need to receive a whole FMCW chirp before processing the FFT, hence, the delay is mostly in the order of 100ms and with a corresponding refresh rate of 10Hz which are both not appropriate for VR/AR applications.

Although previous work has tried to combine the two by statistical methods \cite{xxx} to overcome some of the above problems, no work can address all of those shortcomings.

\begin{figure}
\includegraphics[width=0.5\textwidth]{images/fmcw.png}
\caption{FMCW signal and its demodulation.}
\label{fig:fmcw}
\end{figure}

\subsection{Phase of FMCW signals}

Our key observation is that the phase of the demodulated FMCW signals is also a function of distance. We first formalize the demodulation process.

Let's express the transmitted signal as $$x(t)=exp(-j2\pi (f_0t+\frac{\Delta F}{2T} t^2))$$ where $f_0$ and $\Delta F$ are the initial frequency and bandwidth of the FMCW signal respectively, and $T$ is the duration of the FMCW signal. 
The received signal can be expressed by 

$$y(t)=\sum_{i=1}^M A_iexp(-j2\pi(f_0(t-t_i)+\frac{\Delta F}{2T} (t^2+t_i^2-2tt_i)))$$

where $A_i$ and $t_i=\frac{d_i(t)}{c}$ are the attenuation and received time of the $i$th path transmitted at time $t$. Demodulating this by dividing the original chirp in time domain, we get 

\begin{align}
\hat{y}(t)&=\sum_{i=1}^M A_iexp(-j2\pi (\frac{\Delta F}{T}t_it+f_0t_i-\frac{\Delta F}{2T}t_i^2)) \nonumber\\
&=\sum_{i=1}^M A_iexp(-j(2\pi \mathbf{f}(t_i)t+\mathbf{\phi}(t_i)))
\label{eq:fmcwdemod}
\end{align}

Let's first ignore the multipaths and leave only direct path (say $i=1$).
The initial phase at $t=0$ is then equal to 

\begin{equation}
\mathbf{\phi}_{t_i}(0)=-2\pi(f_0t_i-\frac{\Delta F}{2T}t_i^2)
\label{eq:phasequadratic0}
\end{equation}

Similarly, the phase at $t$ can be expressed by 

\begin{equation}
\mathbf{\phi}_{t_i}(t)=-2\pi(\frac{\Delta F}{T}tt_i+f_0t_i-\frac{\Delta F}{2T}t_i^2)
\label{eq:phasequadratic}
\end{equation}

By solving this quadratic equation, we can get an instantaneous estimate of $t_i$ for each $t$ \footnote{There are two solutions to this quadratic equation, while the other one is out of the range $[0, T]$.}:

\begin{equation}
t_i(t)=\frac{-2\pi(\frac{\Delta F}{T}t+f_0)+\sqrt{4\pi^2(\frac{\Delta F}{T}t+f_0)^2+4\pi\frac{\Delta F}{T}\phi_{t_i}(t)}}{-2\pi\frac{\Delta F}{T}} \label{eq:quadraticsolution}
\end{equation}

Finally the distance can be solved by $d(t)=ct_i(t)$.

Firstly, the ability to get an instantaneous $t_1$ estimate reduces the latency. 
More importantly, the essential property of this method is, with the existence of indirect paths, as long as the sum of the indirect paths has lower amplitude than the direct path, \textit{the $t_1$ estimate using the phases can be approximately 10x more accurate than using the peak in the frequency domain alone}.
We prove it here.


\begin{figure}
\includegraphics[width=0.25\textwidth]{images/phase_err.png}
\caption{Phase error when one indirect path is combined with the direct path.}
\label{fig:phaseerror}
\end{figure}

Suppose the direct path has an amplitude of $A_1$ and time of arrival of $t_1$, one nearby indirect path with amplitude $A_2<A_1$ lies on frequency $\mathbf{f}(t_2)$ in Equation~\ref{eq:fmcwdemod} ($|\mathbf{f}(t_1)-\mathbf{f}(t_2)|<1$). The two peaks will merge together in the frequency domain and will result in a single peak at approximately $(A_2\mathbf{f}(t_2)+A_1\mathbf{f}(t_1))/(A_2+A_1)$ using quadratic interpolation\cite{quadratic_interpolation}. Hence, an frequency error of $(A_2\mathbf{f}(t_2)+A_1\mathbf{f}(t_1))/(A_2+A_1)-\mathbf{f}(t_1)$ which is equivalent to a distance error of 
\begin{equation}
\delta d_{peak}=((A_2\mathbf{f}(t_2)+A_1\mathbf{f}(t_1))/(A_2+A_1)-\mathbf{f}(t_1))*\frac{2c}{\Delta F}
\label{eq:disterr1}
\end{equation}
When we use the phase, the same indirect path would lead to a bounded phase error of $sin^{-1}(\frac{A_2}{A_1})$ (Fig~\ref{fig:phaseerror}) in the worst case. By the Equation~\ref{eq:quadraticsolution}, we can estimate an distance error of 
\begin{equation}
\delta d_{phase}\approx \frac{cos^{-1}(\frac{A_2}{A_1})*c}{2\pi(f_0-\Delta F/8)}
\label{eq:disterr2}
\end{equation}
when $t_1$ is approximate to $T/4$. 

\begin{figure}
\includegraphics[width=0.5\textwidth]{images/errorcompare.eps}
\caption{Error comparison of using the peak vs. our method.}
\label{fig:errcompare}
\end{figure}

We plot the two errors with regard with $A_2/A_1$ and $|\mathbf{f}(t_2)-\mathbf{f}(t_1)|$ in Fig.~\ref{fig:errcompare}. As we see, the error of using the phase of demodulated FMCW signal is approximately 10x less than using the peak frequency.

We however still need to address several important problems to achieve continuous high accuracy acoustic tracking. 

\subsubsection{Estimate speed along with distance}

Estimating speed is essential for motion tracking. Because we can get instantaneous distance measurements, estimating speed is straightforward. In our implementation, we estimate the instantaneous speed by doing least square linear regression of the distances in a 10ms range to reduce the affect from noise and residual multipaths. Note that the least square linear regression in 1D domain is a linear algorithm.

\subsubsection{Large multipath filtering}

The assumption that the sum of indirect paths has lower amplitude than the direct path is too strict. We first need to filter out large multipaths before extracting the phase. Thanks to the property of FMCW signals, we can filter out most multipaths far from the direct paths. We first extract the first peak of the demodulated signal (Equation~\ref{eq:fmcwdemod}), then we apply a linear FIR filter that only leaves a small range of frequency bands around the peak. Note that the taps of the FIR filter need to carefully chosen: if it is too small, it won't have much filtering capability; if it is too large, it will introduce more delay. We set it to an equivalent of 7.5ms delay.

For the $i+1$th chirp, instead of finding peak in the FFT result, we can infer the new peak from the distance and speed estimated from the $i$th chirp, since the latter is far more accurate than the peak of the FFT result. We can further reduce the width of the pass band to filter out more multipath because of this. 

Doppler effect will blur the peak in the frequency domain. We can dynamically increase the width of the pass band of the FIR filter when the speed estimate of previous chirp exceeds a given threshold.
In our implementation, we set the pass band width to $0Hz$ when the speed does not exceed $1m/s$; otherwise, we set the pass band width to $2Hz$. 

\subsubsection{Ambiguity removal and high motion speed support}

Even though we can get the distance and speed from the phase, the phase we get from the demodulated signal is still ambiguous since it is still confined in $[0, 2\pi]$. 
We address this limitation by continuous tracking.
\textit{First chirp}. At the very beginning we assume no motion happens so that we can get an coarse estimate of the distance from the clear peak of the FFT result, denoted by $D$. We also get the ambiguous initial phase $p$ of the filtered demodulated signal. Given the relationship between the distance and the initial phase, we find the best $2N\pi$ added into the ambiguous phase which minimizes the differences of the two measurements $|D-d_{\phi(t=0)=p+2N\pi}(t=0)|$.

\textit{During each chirp}. The phase at each $t$ can be continuously tracked by determining the points where a $2\pi$ cycle ends, where two adjacent phase measurements have a difference more than $\pi$. Note that because the phase error caused by residual indirect paths never exceeds $\pi/2$ throughout each chirp (see Equation~\ref{eq:disterr2}), it will not cause errors during continuous tracking.

\textit{Initial phase of the chirps other than first chirp}. For chirp $i+1$, similar to the FIR filter, given the distance $d^{(i)}(t=T)$ and speed $v^{(i)}(t=T)$ estimated from the end of the previous chirp, we infer the distance estimate of the beginning of the current chirp  $\hat{d}^{(i+1)}(t=0)=d^{(i)}(t=T)+v^{(i)}(t=T)\delta T$. We then find the $2N\pi$ offset in addition to the ambiguous initial phase $p$ that minimize the difference $|d^{(i+1)}_{\phi(t=0)=p+2N\pi}(t=0)-\hat{d}^{(i+1)}(t=0)|$. This in fact transform the constraints of speed in most previous works to a constraint of acceleration, which is much more easier to be satisfied.
Note that each $2\pi$ difference of the phase at any $t<T$ corresponds to an approximately $1.7$cm distance difference. The gap between two adjacent chirp is set to $\delta T=10ms$ in our implementation to eliminate any audible artifacts. Hence, as long as the acceleration does not exceed $85m/s^2$, which is an extreme large number, it will not introduce erroneous offset estimate.
 
\subsubsection{Clock synchronization}

Clock difference exists in any distributed tracking system that causes slow drifts along time. We however use a simple solution to address the problem taking advantage of our extremely accurate distance measurement. At the very beginning, we let the user keep the pair of devices still. The transmitter first transmit the FMCW signal to the receiver. We then let the receiver transmits the same FMCW chirp back to the transmitter. The transmitter does the same distance measurement as the receiver and obtains a distance and speed measurement. Note that the two speed, minus the actual speed (which is zero), are opposite to each other, and the difference is exactly caused by the clock difference and is linear to the clock difference. Estimating the drift which is half the distance difference in unit time, we can then compensate the clock difference by removing the drift for the following measurements. 

\subsection{From 1D to 3D}


\begin{figure}
\includegraphics[width=0.4\textwidth]{images/aoa.png}
\caption{Computing angle of arrival from distance difference.}
\label{fig:fmcw}
\end{figure}

We can extract sub-mm level 1D distance from the above methods, but to get 3D location, we have to solve the two angles in the other two dimensions as well.
Instead of using three or more distanced basestations and solve the intersection of three independent distance measurements, we integrate four microphones in a $15cm\times 10cm$ space so that it can fit in any AR/VR glasses. 
We can infer the two angles from the distance differences from two adjacent microphones. As shown in Fig.~\ref{fig:aoa}, the angle $\alpha=sin^{-1}(\frac{\delta d}{S})$ where $S$ is the separation of the two microphones. 

However, the accuracy of the location on the other two dimensions is also magnified in an order of $\frac{d}{S}$. 
We improve the accuracy by doing an average of the distance differences within each 10ms. Since angular speed (up to a few degrees per 10ms) is not as high as 1D speed in the phase domain (up to a hundred of degrees per 10ms), doing the average will not affect the accuracy during motion. Effectively, this reduces jitters caused by noise as well as biases caused by residual indirect paths.




==> sections/design_1.tex <==
\section{Sub-mm level 1D motion tracking}

Our key contribution to enable the above applications is a novel algorithm pipeline to achieve sub-mm level 1D motion tracking. We use acoustic signals that can be emitted and received by cheap microphone and speaker components or smartphones and smart watches. 

At a high level, our algorithm achieves sub-mm level tracking accuracy by solving the instantaneous phase of the signal meanwhile rejecting indirect multipaths. 
The speaker transmits an inaudible sound signal at a frequency range of 17.5-23.5kHz. The microphone receives the acoustic signal samples which are passed through our algorithms in real time. The precise 1D distance measurement can be computed in a delay as short as 15ms.  

In the rest of this section, we first provide an overview of previous motion tracking methods. We then propose our algorithms to reduce the error by approximately 10x meanwhile supporting high motion speed.  
Thanks to the high 1D accuracy, we use a simple calibration prior to the actual usage to address the synchronization problem.

%To avoid catastrophic errors due to occlusions or noises, we also design a classification method to reset the states when failure happens.

%

% The hardware setup is shown in Fig.~\ref{fig:setup}. A \textit{gadget receiver} consists of one speaker and four microphones sitting on four corners in a $15cm\time 10cm$ rectangle. A \textit{transmitter}, which can be another gadget receiver, a smartphone, or a customized device, requires one speaker and one microphone embedded.


\begin{figure}
\includegraphics[width=0.3\textwidth]{images/setup.png}
\caption{Hardware setup of \name.}
\label{fig:setup}
\end{figure}

% We first review two traditional motion tracking methods.

\subsection{Phase Tracking}

The state-of-the-art acoustic tracking system using phase tracking is SoundTrak\cite{zhang2017soundtrak}.
The transmitter transmit a sine wave $x(t)=exp(-j2\pi ft)$. When there is no multipath, the receiver will receive a delayed signal $y(t)=exp(-j2\pi f(t-\frac{d(t)}{c}))$ where $d(t)$ is the distance between the pair at time $t$, and $c$ is the speed of sound.

The receiver can then downsample the signal by multiplying the carrier wave 
\begin{align}
\hat{y}(t)&=exp(-j2\pi f(t-\frac{d(t)}{c})+j2\pi ft) \nonumber\\
&=exp(j2\pi f\frac{d(t)}{c})
\label{eq:phasetracking}
\end{align}
We can then get the instantaneous phase of it for each $t$ to track the distance $d(t)$. 
Phase tracking is sensitive as a small as 1.6cm displacement would lead to a $2\pi$ phase change. It also introduces negligible delay which only depends on the band pass filter.

However, there are two major problems of this method. Firstly, there exist ambiguity in the phase, \textit{i.e.}, the phase we get from the signal $\phi(t)=(2\pi f\frac{d(t)}{c}) \text{mod} 2\pi$. Because of the modulus operation, we can only get the relative motion but not the absolute distance.
Secondly, when multipath exists, it will lead to severe interference to the combined phase. Single sine wave has no capability to separate multipath. Huge error can be introduced even with the existence of one indirect path. Previous works mitigate this problem by either using multiple frequencies \cite{LLAP}, or introducing sparsity constraint \cite{singleAPWifi}, but it can either only statistically reduce the error linearly to the limited number of frequencies, or requires huge computation of iterative approximated algorithms. 



\subsection{FMCW Tracking}

Another method is to use linear Frequency Modulated Continuous Wave (FMCW) signals (Fig~\ref{fig:fmcw}). The state-of-the-art acoustic tracking system using FMCW is CAT\cite{mao2016cat}. 
Thanks to the good autocorrelation property of FMCW chirps, the receiver is able to differentiate different time-of-arrivals from a single received chirp. For linear FMCW signal, receiver can first demodulate by multiplying the same chirp in the time domain, pass through a low-pass filter, doing FFT and find the peak (Fig~\ref{fig:fmcw}) location, which is linear to the distance. 

Despite most of multipaths can be separated out because of the property of FMCW signals, FMCW tracking has four major shortcomings. Firstly, it does not have a good sensitivity because the precision is limited by the sampling rate and FFT bins, which does not scale computationally. Secondly, indirect paths cannot be totally removed, as nearby paths with a distance separation of less than $O(\frac{c}{2B})$ would merge with the direct path and cause peak deviations. Third, Doppler effect caused by high speed motion can blur the FFT result meanwhile introducing an additional bias to the peak estimate. 
Last but not the least, receiver need to receive a whole FMCW chirp before processing the FFT. This leads to a large delay and a small refresh rate which are both not appropriate for VR/AR applications.

% Although previous work has tried to combine the two by statistical methods \cite{xxx} to overcome some of the above problems, no work can address all of those shortcomings.

\begin{figure}
\includegraphics[width=0.5\textwidth]{images/fmcw.png}
\caption{FMCW signal and its demodulation.}
\label{fig:fmcw}
\end{figure}

\subsection{Phase of Demodulated FMCW signals}

Our key observation is that the phase of the demodulated FMCW signals is also a function of distance. To understand, we first formalize the demodulation process.

Let's express the transmitted signal as $$x(t)=exp(-j2\pi (f_0t+\frac{\Delta F}{2T} t^2))$$ where $f_0$ and $\Delta F$ are the initial frequency and bandwidth of the FMCW signal respectively, and $T$ is the duration of the FMCW signal. 
The received signal can be expressed by 

$$y(t)=\sum_{i=1}^M A_iexp(-j2\pi(f_0(t-t_i)+\frac{\Delta F}{2T} (t^2+t_i^2-2tt_i)))$$

where $A_i$ and $t_i=\frac{d_i(t)}{c}$ are the attenuation and received time of the $i$th path transmitted at time $t$. Since the receiver does not know the exact transmission time at the transmitter side, it introduce a \textit{pseudo chirp} which is the transmitted original chirp with an unknown delay. 
To simplify, we now assume the delay is 0 and will address this synchronization problem later. 
Demodulating the received signal by dividing the pseudo chirp in time domain, we get 

\begin{align}
\hat{y}(t)&=\sum_{i=1}^M A_iexp(-j2\pi (\frac{\Delta F}{T}t_it+f_0t_i-\frac{\Delta F}{2T}t_i^2)) \nonumber\\
&=\sum_{i=1}^M A_iexp(-j(2\pi \mathbf{f}(t_i)t+\mathbf{\phi}(t_i)))
\label{eq:fmcwdemod}
\end{align}

Instead of estimating the peak of the above signal to estimate the time of arrival, we apply a band-pass filter around the peak first to filter out most multipaths. Then we investigate into the instantaneous phase of the filtered signal.

The initial instantaneous phase at $t=0$ is approximate to 

\begin{equation}
\mathbf{\phi}(0)\approx -2\pi(f_0t_d-\frac{\Delta F}{2T}t_d^2)
\label{eq:phasequadratic0}
\end{equation}

where $t_d$ is the time of arrival of the direct path. Similarly, the instantaneous phase at $t$ can be expressed by 

\begin{equation}
\mathbf{\phi}(t) \approx -2\pi(\frac{\Delta F}{T}tt_d+f_0t_i-\frac{\Delta F}{2T}t_d^2)
\label{eq:phasequadratic}
\end{equation}

While we can only get the phase modulo $2\pi$ from the signal ($\hat{\phi}(t)=\mathbf{\phi}(t)\text{ mod }2\pi$), we now assume we know the initial phase offset $2N\pi$; When the phase modulo $2\pi$ appears a sudden jump (\textit{i.e.}, more than $\pi$) between two adjacent $t$ ($t$ and $t-\delta t$), we know there is a $2\pi$ jump at that time:

\begin{align}
\mathbf{\Delta \phi}(0)= & 0 \nonumber \\
\mathbf{\Delta \phi}(t)=&-2\pi+\mathbf{\Delta \phi}(t-\delta t), &\text{if } \hat{\phi}(t)-\hat{\phi}(t-\delta t)>\pi \nonumber \\
& 2\pi+\mathbf{\Delta \phi}(t-\delta t), &\text{if } \hat{\phi}(t)-\hat{\phi}(t-\delta t)<-\pi \nonumber \\
& \mathbf{\Delta \phi}(t-\delta t), &\text{otherwise} \nonumber \\
\mathbf{\phi}(t) \approx & 2N\pi+ \hat{\phi}(t)+\mathbf{\Delta \phi}(t)
\label{eq:phaseambiguity}
\end{align}


By solving this quadratic equation, we can get an instantaneous estimate of $t_d$ for each $t$ \footnote{There are two solutions to this quadratic equation, while the other one is out of the range $[0, T]$.}:

\begin{equation}
t_d(t) \approx \frac{-2\pi(\frac{\Delta F}{T}t+f_0)+\sqrt{4\pi^2(\frac{\Delta F}{T}t+f_0)^2+4\pi\frac{\Delta F}{T}\phi(t)}}{-2\pi\frac{\Delta F}{T}} \label{eq:quadraticsolution}
\end{equation}

Finally the distance can be solved by 
\begin{equation}
    d(t)=ct_d(t)
    \label{eq:quadraticsolutiond}
\end{equation}

The essential property of this method is, with the existence of unfiltered indirect paths, as long as the sum of the indirect paths has lower amplitude than the direct path, \textit{the $t_1$ estimate using the phases can be approximately 10x more accurate than using the peak estimate in the frequency domain alone}.
We prove it here.

\begin{proof}

\begin{figure}
\includegraphics[width=0.25\textwidth]{images/phase_err.png}
\caption{Phase error when one indirect path is combined with the direct path.}
\label{fig:phaseerror}
\end{figure}

Suppose the direct path has an amplitude of $A_1$ and time of arrival of $t_1$, one nearby indirect path with amplitude $A_2<A_1$ lies on frequency $\mathbf{f}_{t_2}$ in Equation~\ref{eq:fmcwdemod} ($|\mathbf{f}_{t_1}-\mathbf{f}_{t_2}|<1$). 
The two peaks will merge together in the frequency domain resulting in a single peak at approximately $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)$ using quadratic interpolation\cite{quadratic_interpolation}. Hence, a frequency error of $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)-\mathbf{f}_{t_1}$ which is equivalent to a distance error of 
\begin{equation}
\delta d_{peak}=(\frac{A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1}}{A_2+A_1}-\mathbf{f}_{t_1})*\frac{2c}{\Delta F}
\label{eq:disterr1}
\end{equation}
When we use the phase, the same indirect path would lead to a bounded phase error of $sin^{-1}(\frac{A_2}{A_1})$ (Fig~\ref{fig:phaseerror}) in the worst case. 
Because of this error is bounded in $(-\pi/2, \pi/2)$, the error will not cause a more than $\pi$ jump in Equation~\ref{eq:phaseambiguity} so it will not cause errors within a chirp. 

To simplify the analysis, we assume $t_d\approx T/4$. Note that we can always time-shift the pseudo chirp during processing in order to make $t_d$ fall into a reasonable range. 
From Equation~\ref{eq:quadraticsolution}, we can estimate an distance error of 
\begin{equation}
\delta d_{phase}\approx \frac{cos^{-1}(\frac{A_2}{A_1})*c}{2\pi(f_0-\Delta F/8)}
\label{eq:disterr2}
\end{equation}
during each chirp. 

\begin{figure}
\includegraphics[width=0.5\textwidth]{images/errorcompare.eps}
\caption{Error comparison of using the peak vs. our method.}
\label{fig:errcompare}
\end{figure}

We plot the two errors with regard with $A_2/A_1$ and $|\mathbf{f}(t_2)-\mathbf{f}(t_1)|$ in Fig.~\ref{fig:errcompare}. As we see, the error of using the phase of demodulated FMCW signal is in the order of 10x less than using the peak frequency.
\end{proof}

We however still need to address several important problems to achieve continuous high accuracy acoustic tracking. 

\subsubsection{Estimate speed along with distance}

Estimating speed is essential for motion tracking. It is also the key to our system to achieve reliable tracking. 
Because we can get instantaneous distance measurements, estimating speed is straightforward. In our implementation, we estimate the instantaneous speed by doing least square linear regression of the distances in a 10ms range to reduce the affect from noise and residual multipaths. Note that the least square linear regression in 1D domain is a linear algorithm.

\subsubsection{Phase ambiguity removal}

Even though we can get the distance and speed from the phase, there is still one unsolved problem: the initial $2N\pi$ phase offset during the demodulation of each chirp.  
We address this limitation by continuous tracking.

\textbf{First chirp}. At the very beginning we assume no motion happens so that we can get an coarse estimate of the distance from the clear peak of the FFT result, denoted by $D$. We also get the ambiguous initial phase $\hat{\phi}(0)$ of the filtered demodulated signal. Given the relationship between the distance and the initial phase, we find the best $2N\pi$ added into the ambiguous phase which minimizes the differences of the two measurements $|D-d_{\phi(0)=\hat{\phi}(0)+2N\pi}(0)|$ (Equation~\ref{eq:quadraticsolutiond}).

\textbf{Chirps other than first chirp}. For chirp $i+1$, given the distance $d^{(i)}(t=T)$ and speed $v^{(i)}(t=T)$ estimated from the end of the previous chirp, we can infer the distance estimate of the beginning of the current chirp  $\hat{d}^{(i+1)}(t=0)=d^{(i)}(t=T)+v^{(i)}(t=T)\delta T$. We then find the $2N\pi$ offset in addition to the ambiguous initial phase $\hat{\phi}(0)$ that minimize the difference $|d^{(i+1)}_{\phi(0)=\hat{\phi}(0)+2N\pi}(0)-\hat{d}^{(i+1)}(t=0)|$. 
This in fact relaxes the constraints of velocity in most previous works to a constraint of acceleration, which is much more easier to be satisfied.
Note that each $2\pi$ difference of the phase at any $t<T$ corresponds to an approximately $2$cm distance difference. Hence, any error smaller than $1$cm will not cause an erroneous estimate. The gap between two adjacent chirp plus the delay caused by the band-pass filter is approximately $\delta T=15ms$ in our implementation. Hence, as long as the acceleration does not exceed $44m/s^2$, which is an extreme large number, it will not introduce erroneous offset estimate.

\subsubsection{Adaptive band-pass filter configuration}

During the processing, we first extract the first peak of the demodulated signal (Equation~\ref{eq:fmcwdemod}), then we apply a linear FIR filter that only leaves a small range of frequency bands around the peak. The delay of the FIR filter need to carefully chosen: if it is too small, it won't have much filtering capability, thus leaving noise and residual indirect paths; if it is too large, it will introduce more delay and more gap between two chirps, reducing the maximum supported acceleration.

We adaptively set the delay of the FIR filter from the SNR. In our configuration, when $SNR<10dB$, we use a 15ms delay; otherwise, we reduce the delay to $7.5ms$.

For the $i+1$th chirp, instead of finding peak in the FFT result, we can infer the new peak from the distance and speed estimated from the $i$th chirp, since the latter is far more accurate than the peak of the FFT result. 

Doppler effect will blur the peak in the frequency domain. Similarly, we can adaptively increase the width of the pass band of the FIR filter when the speed estimate of previous chirp exceeds a given threshold.
In our implementation, we set the pass band width to $1Hz$ when the speed does not exceed $1m/s$; otherwise, we set the pass band width to $2Hz$. 

\subsection{Clock Synchronization}

Clock difference exists in any distributed tracking system that causes a) unknown starting point; and b) slow drifts along time. We however use a simple calibration to address the problem taking advantage of our accurate distance measurement. 

At the very beginning, we let the user to touch the speaker in the transmitter with the microphone in the receiver. 
%The transmitter first transmit the FMCW signal to the receiver. We then let the receiver transmits the same FMCW chirp back to the transmitter. The transmitter does the same distance measurement as the receiver and obtains a distance and speed measurement. Note that the two speed, minus the actual speed (which is zero), are opposite to each other, and the difference is exactly caused by the clock difference and is linear to the clock difference. 
We meanwhile start the above algorithm to estimate the distance for 5 seconds. 
Because of the clock difference, the receiver can detect a constant moving speed which is linear to the clock difference. We can then compensate the clock difference by removing the drift for the following measurements at the receiver side. 
We also set the time offset of the pseudo chirp so that the measured distance between the two devices at the end of the calibration is zero, so that we can get the absolute distance measurements for the following usages.


\subsection{Concurrent Transmission Support}

Because of the one-way transmission nature of the above algorithm, \name support concurrently tracking arbitrary number of microphones with regard to one speaker at the same time.
Even better, we can support concurrent transmissions from multiple speakers to single microphone as well. 

Our insight is that the receiver can regard transmissions from other transmitters as multipath. Thus, they are filtered out by the band-pass filter at the first step.

Let's take the application of finger ring tracking as example. At the beginning, five finger rings coordinate with each other so that the $i$th finger ring introduces a $iT/20$ starting time offset of the chirps it emits. 
The receiver demodulate the received signals and there exist five separate peaks in the frequency domain, where the $i$th peak corresponds to the $i$th finger ring.

It can then track each of them using five different band-pass filters without losing accuracy nor agility. Note that if two peaks merge together the receiver would not track either of them, but for the finger rings tracking, the distance between two finger rings would never exceeds the threshold of peak merging (about 1m).

\section{From 1D to 3D}

\begin{figure}
\includegraphics[width=0.4\textwidth]{images/aoa.png}
\caption{Computing angle of arrival from distance difference.}
\label{fig:fmcw}
\end{figure}

We can extract accurate level 1D distances from the above methods. 
To get 3D location, we need to use the information from at least three 1D measurements.
Instead of using multiple speakers, we use multiple microphones at the receiver side to reduce the power consumption. 

Thanks to the accurate 1D measurements, we can shrink the separation between microphones to as small as a few centimeters meanwhile still keeping an acceptable accuracy. The microphone array can even be embedded in a pocket-able device.   

Specifically, we place four microphones at four corners of a rectangle. 
Assuming the axis perpendicular to the microphone array plane as $x$. We can infer the 2D positions in $x-y$ (or $x-z$) plane from the intersection from one of the two vertical (horizontal) microphone pair. As shown in Fig.~\ref{fig:aoa}, TODO

However, using this method, the accuracy of the location on the $y$ and $z$ axis is also magnified in an order of $\frac{d}{S}$ where $d$ is the distance between the microphone array and speaker. 
We improve the accuracy by doing an average of the distance measurements within each 10ms. Since angular speed (up to a few degrees per 10ms) is not as high as 1D speed in the phase domain (up to a hundred of degrees per 10ms), doing the average will not affect the accuracy during motion. Effectively, this reduces jitters and improves user experience.
 
\section{Failure Detection and Recovery}

Our accurate localization accuracy relies on continuous tracking. When tracking failure happens, the subsequent measurements are also prone to errors. As a result, a failure detection mechanism is necessary. 
In practice, tracking failures are due to two reasons: a) occlusions; and b) noises.  

\subsubsection{Failures due to occlusion}

Acoustic signal can penetrate some occlusions such as fabrics and , but for other types of occlusions like wood and human limbs, refraction between different transmission mediums causes a dense multipath around the
direct path which is also greatly attenuated. Therefore, the above algorithm fails because it doesn't satisfy the premise that the direct path dominates the filtered demodulated signal. 

When the error happens during a chirp, it will cause fluctuations during the phase tracking(Fig~\ref{fig:occlusionerror1}) because two or more similar frequencies destruct and enhance the amplitudes at different times; When the error happens between two chirps, it will lead to wrong $2N\pi$ estimate that causes a $~2cm$ error for the subsequent chirps.

To detect, in the first situation, we set the constraint of acceleration and the phase fluctuations will cause rapid distance fluctuation as well as a huge acceleration that exceeds the constraints; In the second situation, because we have four microphones, it is very unlikely that the four encounter the same error at the same time because of their different locations. Hence, if the measurements from some of the four microphones are suddenly $2cm$ off the measurements from the others, it indicates an measurement error. 

\subsubsection{Failures due to noise}

Noise can be easily measured by SNR, which can be calculated from the raw demodulated signal prior to the band-pass filter. A low SNR results in noisy phase measurements. Similar to the above scenarios, it is prone to a wrong $2N\pi$ estimate and can be detected by the anomalies of the measurements from four microphones.

\subsubsection{Recovery}

When failure is detected, the receiver falls back to the traditional peak estimation method for FMCW signals. When the signs of the failure disappear, the receiver will notify the user to stop movement to re-calculate the $2N\pi$ and resume accurate measurements.


==> sections/design_2.tex <==
\section{Sub-mm level 1D motion tracking}

Our key contribution to enable the above applications is a novel algorithm pipeline to achieve sub-mm level 1D motion tracking. We use acoustic signals that can be emitted and received by cheap microphone and speaker components or smartphones and smart watches. 

At a high level, our algorithm achieves sub-mm level tracking accuracy by solving the instantaneous phase of the signal meanwhile rejecting indirect multipaths. 
The speaker transmits an inaudible sound signal at a frequency range of 17.5-23.5kHz. The microphone receives the acoustic signal samples which are passed through our algorithms in real time. The precise 1D distance measurement can be computed in a delay as short as XXms.  

In the rest of this section, we first describe our proposed distance estimation algorithms to reduce the error by approximately 10x; We then provide solutions to address the phase ambiguity and clock synchronization problem. Finally, we design adaptive methods to support long range and high motion speed.  

%To avoid catastrophic errors due to occlusions or noises, we also design a classification method to reset the states when failure happens.

%

% The hardware setup is shown in Fig.~\ref{fig:setup}. A \textit{gadget receiver} consists of one speaker and four microphones sitting on four corners in a $15cm\time 10cm$ rectangle. A \textit{transmitter}, which can be another gadget receiver, a smartphone, or a customized device, requires one speaker and one microphone embedded.


\begin{figure}
\includegraphics[width=0.3\textwidth]{images/setup.png}
\caption{Hardware setup of \name.}
\label{fig:setup}
\end{figure}

% We first review two traditional motion tracking methods.

\subsection{FMCW Tracking}

The basic intuition of tracking methods is to track the changing time-of-arrival of the transmitted signals at the receiver side. 
The simplest signal we can use is a sine signal, \textit{i.e.}, $x(t)=exp(-j2\pi ft)$ where $f$ is the wave frequency, and the receiver obtains its changing phase to estimate the changing time-of-arrival $t_d$: $\hat{y}(t)=exp(-j2\pi f(t-t_d)+j2\pi ft)=exp(j2\pi ft_d)$.
However, with the existance of multipath, severe interference leads to a combined distorted phase where one cannot separate each paths. % The ambiguity of the phase because of its $2\pi$ cycle makes it unable to recover from erroneous results.  

To combat with multipath, linear Frequency Modulated Continuous Wave (FMCW) signals (Fig~\ref{fig:fmcw}) can be used
thanks to its good autocorrelation property. 
The receiver is able to differentiate different time-of-arrivals from a single received chirp. 
Specifically, let's express the transmitted FMCW chirp as $$x(t)=exp(-j2\pi (f_0t+\frac{B}{2T} t^2))$$ where $f_0$ and $B$ are the initial frequency and bandwidth of the FMCW chirp respectively, and $T$ is the duration of the FMCW signal. 
The received signal can be expressed by 

$$y(t)=\sum_{i=1}^M A_iexp(-j2\pi(f_0(t-t_i)+\frac{B}{2T} (t^2+t_i^2-2tt_i)))$$

where $A_i$ and $t_i=\frac{d_i(t)}{c}$ are the attenuation and received time of the $i$th path transmitted at time $t$. Since the receiver does not know the exact transmission time at the transmitter side, it instead uses a \textit{pseudo chirp} which is a virtual FMCW chirp with an unknown delay to the transmitted signal. The unknown delay would introduce a constant distance offset to the final result and can be corrected by a synchronization method we will discuss later.
We here assume the delay is 0 for simplification.

Demodulating the received signal by dividing the pseudo chirp in time domain, we get 

\begin{align}
\hat{y}(t)&=\sum_{i=1}^M A_iexp(-j2\pi (\frac{B}{T}t_it+f_0t_i-\frac{B}{2T}t_i^2)) \label{eq:fmcwdemod}
\end{align}


We see that distanced multipath fall into different frequencies. The receiver then use FFT to obtain its frequency domain and find the first peak (Fig~\ref{fig:fmcw}) location, which is linear to the distance of the direct path:

\begin{equation}
    d(t)=\frac{cf_{peak}}{B}
    \label{eq:peaksolutiond}
\end{equation}

However, indirect paths still affects the accuracy because of the small bandwidth. With a bandwidth $B$ and $c$ as speed of sound, paths near the direct path with a distance difference of less than $O(\frac{c}{2B})$ would merge with the direct path in the frequency domain and cause result deviations which, in our scenario, is in the order of centimeters. 
Worse, Doppler effect caused by high speed motion can blur the frequency domain meanwhile introducing an additional bias in the order of $XXX$ to the peak estimate, which translates to a XXcm error when the motion speed is $1m/s$. 
The nature of FFT also limits the agility, because the receiver needs to receive the whole chirp before doing the FFT in order to achieve the best performance. 


\begin{figure}
\includegraphics[width=0.5\textwidth]{images/fmcw.png}
\caption{FMCW signal and its demodulation.}
\label{fig:fmcw}
\end{figure}

\subsection{Phase of Demodulated FMCW signals}

Our intuition is that besides the frequency, the phase of the demodulated FMCW signals is also a function of the distance. 

Instead of using the first peak frequency of the demodulated FMCW signal to estimate the time-of-arrival, we apply a narrow band-pass filter around the first peak to filter out most multipath. This leaves us only a small portion of residual indirect paths around the direct path. Then we investigate into the instantaneous phase of the filtered signal.

From Eq.~\ref{eq:fmcwdemod}, the initial instantaneous phase at $t=0$ is approximate to 

\begin{equation}
\mathbf{\phi}(0)\approx -2\pi(f_0t_d-\frac{B}{2T}t_d^2)
\label{eq:phasequadratic0}
\end{equation}

where $t_d$ is the time of arrival of the direct path. The approximation is due to the residual indirect paths and noise. Similarly, the instantaneous phase at $t$ can be expressed by 

\begin{equation}
\mathbf{\phi}(t) \approx -2\pi(\frac{B}{T}tt_d+f_0t_d-\frac{B}{2T}t_d^2)
\label{eq:phasequadratic}
\end{equation}

By solving this quadratic equation, we can get an instantaneous estimate of $t_d$ for each $t$ from the instantaneous phase$\phi(t)$ \footnote{There are two solutions to this quadratic equation, while the other one is out of the range $[0, T]$.}:

\begin{equation}
t_d(t, \phi(t)) \approx \frac{-2\pi(\frac{B}{T}t+f_0)+\sqrt{4\pi^2(\frac{B}{T}t+f_0)^2+4\pi\frac{B}{T}\phi(t)}}{-2\pi\frac{B}{T}} \label{eq:quadraticsolution}
\end{equation}

Finally the distance can be solved by 
\begin{equation}
    d(t, \phi(t))=ct_d(t, \phi(t))
    \label{eq:quadraticsolutiond}
\end{equation}

The key observation is that the distance derived from the phase using Eq.~\ref{eq:quadraticsolutiond} is much more sensitive than then distance derived from the frequency peak using Eq.~\ref{eq:peaksolutiond}. Specifically, we state that

\begin{theorem}
With the existence of unfiltered indirect paths, as long as the sum of the indirect paths has lower amplitude than the direct path, the error of the $d(t)$ estimate using the Eq.~\ref{eq:quadraticsolutiond} is bounded to $\frac{sin^{-1}(A_2/A_1)*c}{2\pi(f_0-B/2)}$ when $A_1$ and $A_2$ are the amplitude of the direct path and the total amplitude of the indirect paths, respectively. 
\end{theorem}
\begin{proof}

\begin{figure}
\includegraphics[width=0.25\textwidth]{images/phase_err.png}
\caption{Phase error when one indirect path is combined with the direct path.}
\label{fig:phaseerror}
\end{figure}

As seen in Fig.~\ref{fig:phaseerror}, the complex representation of the (sum of) indirect paths are added to the complex representation of the direct path, the deviation would lead to a bounded phase error of $sin^{-1}(\frac{A_2}{A_1})$ in the worst case. 

Now we derive the distance error from the phase error.
From Eq.~\ref{eq:phasequadratic}, we regard $t_d$ as another parameter of $\phi$. We know its derivative regarding to $t_d$

$$\frac{d\phi(t, t_d)}{dt_d}=-2\pi(\frac{B}{T}t+f_0-\frac{B}{T}t_d)<0$$
when $t_d<T$. Its second derivative
$$\frac{d^2\phi(t, t_d)}{dt_d^2}=2\pi\frac{B}{T}>0$$
So it is a convex function.

Suppose an phase error $\phi_e$ would introduce a time-of-arrival error of $t_e$. 
Without loss of generality, we assume $\phi_e>0$. we know that for any $t$

\begin{align*}
\phi(t, t_d)&>\phi(t, t_d+t_e)-\frac{d \phi(t, t_d+t_e)}{d t_d}t_e \\
\phi_e&>-\frac{d\phi(t, t_d+t_e)}{dt_d}t_e \\
t_e&<\frac{\phi_e}{-\frac{d\phi(t, t_d+t_e)}{dt_d}} =\frac{\phi_e}{2\pi(\frac{B}{T}t+f_0-\frac{B}{T}(t_d+t_e)}\\
&< \frac{\phi_e}{2\pi(f_0-\frac{B}{T}\frac{T}{2})} \\
&= \frac{sin^{-1}(\frac{A_2}{A_1})}{2\pi(f_0-\frac{B}{2})}
\end{align*}

Hence, the distance error is bounded by

\begin{equation}
d_e^{(phase)}<\frac{sin^{-1}(\frac{A_2}{A_1})*c}{2\pi(f_0-B/2)}
\label{eq:disterr2}
\end{equation}

\end{proof}

\begin{figure}
\includegraphics[width=0.5\textwidth]{images/errorcompare.eps}
\caption{Error comparison of using the peak vs. our method.}
\label{fig:errcompare}
\end{figure}


We compare it to the traditional peak estimation method for FMCW signals. We denote the time-of-arrival of the direct path as $t_1$ and its frequency in the demodulated FMCW signal as $\mathbf{f}_{t_1}$ ; The nearby indirect path with a time-of-arrival of $t_2$ lies at frequency $\mathbf{f}_{t_2}$ in the demodulated signal. When $|\mathbf{f}_{t_1}-\mathbf{f}_{t_2}|<1$, 
the two peaks will merge together in the frequency domain resulting in a single peak at approximately $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)$ using quadratic interpolation\cite{quadratic_interpolation}. Hence, a frequency error of $(A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1})/(A_2+A_1)-\mathbf{f}_{t_1}$ which is equivalent to a distance error of 
\begin{equation}
d_e^{(peak)}=(\frac{A_2\mathbf{f}_{t_2}+A_1\mathbf{f}_{t_1}}{A_2+A_1}-\mathbf{f}_{t_1})*\frac{2c}{B}
\label{eq:disterr1}
\end{equation}


We plot the two errors with regard with $A_2/A_1$ and $|\mathbf{f}(t_2)-\mathbf{f}(t_1)|$ in Fig.~\ref{fig:errcompare}. As we see, the error of using the phase of demodulated FMCW signal is in the order of 10x less than using the peak frequency.



%We however still need to address several important problems to achieve continuous high accuracy acoustic tracking. 


\subsection{Phase Ambiguity Removal}

While the above method suggests a high accuracy potential, like any phase tracking algorithm, we still need to address the problem of phase ambiguity. 
Specifically, 
we can only get the phase modulo $2\pi$ from the demodulated chirp ($\hat{\phi}(t)=\mathbf{\phi}(t)\text{ mod }2\pi$).
Here we need to address two separate phase ambiguity problem: a) how to detect the $2\pi$ shift during one chirp; and b) how to estimate the initial $2N\pi$ phase offset, \textit{i.e.,} $\mathbf{\phi}(0)=2N\pi+\hat{\phi}(0)$.

\subsubsection{Phase ambiguity during the chirp}
When the phase modulo $2\pi$ appears a sudden jump (\textit{i.e.}, more than $\pi$) between two adjacent $t$ (denoted as $t$ and $t-\delta t$), we know there is a $2\pi$ jump at that time:

\begin{align}
\mathbf{\Delta \phi}(0)= & 0 \nonumber \\
\mathbf{\Delta \phi}(t)=&-2\pi+\mathbf{\Delta \phi}(t-\delta t), &\text{if } \hat{\phi}(t)-\hat{\phi}(t-\delta t)>\pi \nonumber \\
& 2\pi+\mathbf{\Delta \phi}(t-\delta t), &\text{if } \hat{\phi}(t)-\hat{\phi}(t-\delta t)<-\pi \nonumber \\
& \mathbf{\Delta \phi}(t-\delta t), &\text{otherwise} \nonumber \\
\mathbf{\phi}(t) \approx & 2N\pi+ \hat{\phi}(t)+\mathbf{\Delta \phi}(t)
\label{eq:phaseambiguity}
\end{align}

Note that the phase error caused by residual indirect paths is bounded in $(-\pi/2, \pi/2)$. Hence, the error will not cause a more than $\pi$ jump in Equation~\ref{eq:phaseambiguity} so it will not cause $2\pi$ errors within a chirp. 


\subsubsection{Phase ambiguity at the beginning of the chirp}

We address the initial phase ambiguity using speculation of the estimated distance given the last measured distance and speed. 

Because we can get instantaneous distance measurements, estimating speed is straightforward. In our implementation, we estimate the instantaneous speed by doing least square linear regression of the distances in a 10ms range to reduce the affect from noise and residual multipaths. Note that the least square linear regression in 1D domain is a linear algorithm.

%Even though we can get the distance and speed from the phase, there is still one unsolved problem: the initial $2N\pi$ phase offset during the demodulation of each chirp.  
%We address this limitation by continuous tracking.

For the $i+1$th received chirp, given the distance $d^{(i)}_{end}$ and speed $v^{(i)}_{end}$ estimated from the end of the $i$th chirp, we can infer the distance of the beginning of the current chirp  $\hat{d}^{(i+1)}_{start}=d^{(i)}_{end}+v^{(i)}_{end}\delta T$ where $\delta T$ is the gap between two chirps. 
We then find the $2N\pi$ offset in addition to the ambiguous initial phase $\hat{\phi}(0)$ that minimize the difference $|d^{(i+1)}(0, \hat{\phi}(0)+2N\pi)-\hat{d}^{(i+1)}_{start}|$. 
This in fact relaxes the constraints of velocity in most previous works to a constraint of acceleration, which is much more easier to be satisfied.
Note that each $2\pi$ difference of the phase at any $t<T$ corresponds to an approximately $2$cm distance difference. Hence, any error smaller than $1$cm will not cause an erroneous $2N\pi$ estimate. The gap between two adjacent chirp plus the delay caused by the band-pass filter is approximately $\delta T=20ms$ in our implementation. Hence, as long as the acceleration does not exceed $25m/s^2$, which is an extremely large number, it will not introduce erroneous offset estimate.



\subsection{Clock Synchronization}

Clock difference exists in any distributed tracking system that causes a) unknown starting point; and b) slow drifts along time. We however use a simple calibration to address the problem taking advantage of our accurate distance measurement. 


At the very beginning, we let the user to touch the speaker in the transmitter with the microphone in the receiver. 
The receiver meanwhile start recording the chirp for 5 seconds and run the above tracking algorithm.


\subsubsection{Estimating the delay of the pseudo chirp}
For the first received chirp, we use autocorrelation to determine a coarse starting time. We set the pseudo chirp starting at the same time.  

\subsubsection{Estimating the initial phase offset}
Because of a high SNR, no motion and little indirect path because of the zero distance, the estimate of the distance from the peak of the FFT result, denoted by $D$, is accurate enough. 
As a result, for the first demodulated chirp, we can find the initial $2N\pi$ phase offset from $D$. Specifically, we find the best $2N\pi$ added into the ambiguous phase which minimizes the differences of the two measurements $|D-d(0, \hat{\phi}(0)+2N\pi)|$.


\subsubsection{Estimating drift}
Because of the clock difference, the receiver can detect a constant moving speed within the 5 seconds which is linear to the clock difference. We can then compensate the clock difference by removing the drift for the following measurements at the receiver side. 


\subsection{Adaptive band-pass filter configuration}

For the first demodulated chirp, we need to extract the first peak of the demodulated signal (Equation~\ref{eq:fmcwdemod}), then apply a FIR filter that only leaves a narrow range of frequency bands around the peak. The delay of the FIR filter need to be carefully chosen: if it is too small, it cannot filter most indirect paths and also leaves a lot of noise; if it is too large, it will introduce more latency and more gap between two chirps, reducing the maximum supported acceleration.

We adaptively set the delay of the FIR filter from the SNR. In our configuration, when $SNR>10dB$, we use a 15ms delay; otherwise, we double the delay to $30ms$.

For the $i+1$th chirp, instead of finding peak in the FFT result, we can infer the new peak from the distance and speed estimated from the $i$th chirp using the same solution to the phase ambiguity problem, since a) it is far more accurate than the peak of the FFT result; and b) it does not requires receiving a whole chirp before processing, thus reducing the latency. 

Doppler effect will blur the peak in the frequency domain. Similarly, we can adaptively increase the width of the pass band of the FIR filter when the speed estimate at the end of the previous chirp exceeds a given threshold.
In our implementation, we set the pass band width to $1Hz$ when the speed does not exceed $1m/s$; otherwise, we set the pass band width to $2Hz$. 



\section{Millimeter Level 3D Motion Tracking}

Based on the 1D motion tracking algorithm, in this section we describe how to achieve a reliable 3D motion tracking.

\begin{figure}
\includegraphics[width=0.4\textwidth]{images/aoa.png}
\caption{Computing angle of arrival from distance difference.}
\label{fig:aoa}
\end{figure}

\subsection{From 1D to 3D}

We can extract accurate level 1D distances from the above methods. 
To get 3D location, we need to use the information from at least three 1D measurements.
Instead of using multiple speakers, we use multiple microphones at the receiver side to reduce the power consumption. 

Thanks to the accurate 1D measurements, we can shrink the separation between microphones to as small as a few centimeters meanwhile still keeping an acceptable accuracy. %The microphone array can even be embedded in a pocket-able device.   

Specifically, we place four microphones at four corners of a rectangle. 
Assuming the axis perpendicular to the microphone array plane as $x$. We can infer the 2D positions in $x-y$ (or $x-z$) plane from the intersection from one of the two vertical (horizontal) microphone pair, as shown in Fig.~\ref{fig:aoa} (\red{need to update}).

However, using this method, the accuracy of the location on the $y$ and $z$ axis is also magnified in an order of $\frac{d}{S}$ where $d$ is the distance between the microphone array and speaker. 
We improve the accuracy by doing an average of the distance measurements within each 10ms. Since angular speed (up to a few degrees per 10ms) with regard to $x$ axis is not as high as 1D speed in the phase domain (up to a hundred of degrees per 10ms), doing the average will not affect the accuracy during motion. Effectively, this reduces jitters and improves the accuracy.
 
\subsection{Failure Detection and Recovery}

Our accurate localization accuracy relies on continuous tracking. When tracking failure happens, the subsequent measurements are also prone to errors. As a result, a failure detection mechanism is necessary. 
In practice, tracking failures are due to two reasons: a) occlusions; and b) noises.  

\subsubsection{Failures due to occlusion}

Acoustic signal can penetrate some occlusions such as fabrics, but for other types of occlusions like wood and human limbs, refraction between different transmission mediums causes a dense multipath around the
direct path which is also greatly attenuated. Therefore, the above algorithm fails because it doesn't satisfy the premise that the direct path dominates the filtered demodulated signal. 

When the error happens during a chirp, it will cause fluctuations during the phase tracking(Fig~\ref{fig:occlusionerror1}) because two or more similar frequencies destruct and enhance the amplitudes at different times. There would be multiple $2\pi$ phase tracking error during the chirp, leading to a larger than $2cm$ distance error at the end of the chirp. When the error happens between two chirps, it will lead to wrong $2N\pi$ estimate that causes a larger than $~2cm$ error for the subsequent chirps.

\subsubsection{Failures due to noise}

On longer ranges the signal attenuates so that the SNR is lower. A low SNR results in noisy phase measurements. Similar to the above scenarios, it is prone to a wrong $2N\pi$ estimate.

\subsubsection{Detection}
We detect failures utilizing the redundancy of the microphones. 
Because we have four microphones, it is very unlikely that the four encounter the same error at the same time because of their different locations. Hence, if the measurements from some of the four microphones are suddenly at least $2cm$ off the measurements from the others, it indicates an error. 



\subsubsection{Recovery}

When failure is detected, if the anomaly is only one microphone, the receiver will first try to compensate the $2\pi$ offset until it is in the similar range of the other three microphones. If continuing failures happen (which rarely happens), it falls back to the traditional peak estimation method for FMCW signals and notify the user.

% move it to the next section
\section{Concurrent Transmissions}

Because of the one-way transmission nature of the above algorithm, \name support concurrently tracking arbitrary number of microphones with regard to one speaker at the same time.
Even better, we can support concurrent transmissions from multiple speakers to single microphone as well, because FMCW chirps with different delays are orthogonal to each other \cite{lora}. 

Our insight is that the receiver can regard transmissions from other transmitters as multipath. Thus, they are filtered out by the band-pass filter at the first step.

At the beginning, $N$ transmitters coordinate with each other using any networking protocol so that the $i$th transmitter introduces a $iT/N$ starting time offset of the chirps it emits. 
The coordination information is also sent to the receivers, which demodulate the received signals. There exist five separate peaks in the frequency domain, where the $i$th peak corresponds to the $i$th transmitter.
It can then track the phase of each of them using five different band-pass filters without losing accuracy nor agility. 

Note that because of motion, if multiple peaks merge together the receiver would not track any of them, so essentially this trades off the working range of each transmitter. 
However, the transmitters and receivers can run the coordination protocol periodically to assign a new evenly distributed starting time offset.


==> sections/intro_0.tex <==
\section{Introduction}

% application background: AR

Augmented Reality (AR) or Mixed Reality (MR), by merging real world with computer-generated virtual world, provides an immersible and authentic virtual environments that Virtual Reality (VR) techniques cannot provide \cite{}. More importantly, AR techniques enable new opportunities of human-computer interactions, where human actions could have a more straight-forward feedback in the merged world.

An essential enabler of such interactions is \textit{wireless controller}. The key two capabilities of such controllers are a) interactions like tapping, pressing, sliding, that users can easily perform by their hands and fingers, and b) their positions can be tracked accurately and instantly without perceivable delay.
While the first capability can be easily fulfilled by dedicated controllers and smartphones, the second capability is challenging and may require extra assisting hardware. 

% ask question

In this paper, we ask the following question: Without any other base-stations, can we turn any smartphone into a sub-millimeter tracking ability wireless controller for AR devices? 
For example, in a painting app our smartphone can act as the pen and we can easily change its color and style by interacting with the virtual palette on the screen of the smartphone; in an AR shooting game we can use our smartphone as weapon and a button on the screen is designed as its trigger; We can also access the inertial sensors inside the smartphone to obtain the rotation in addition to the translation, further enhancing its interaction capabilities.  

% challenges

While there exists wireless controllers that can be tracked in sub-millimeter accuracy for commercial VR glasses \cite{HTC_Lighthouse, Oculus_controller}, few of them can also be adopted to AR glasses. The reason is the fundamental difference between the typical use scenarios between them.

VR devices are mostly used in a confined indoor environments where users have a limited environment to move and interact. 
However, for AR devices, the capability of augmented reality with virtual objects allow users to take with them everywhere they go to enhance their real-world experience. It is not practical to place multiple base stations in fixed and distanced locations anywhere we take AR glasses. While off-the-shelf commercial controllers rely on base stations to measure the time of arrival (ToA) or time difference of arrival (TDoA) and calculating its location by trangulation \cite{}, they are not applicable for AR controllers. 

Secondly, while AR devices can localize themselves by computer vision algorithms like SLAM\cite{} using their cameras, it is computationally extensive to continuously tracking itself, which even requires dedicated hardware accelerator to support real-time processing. Additionally, computer vision solutions fail at low refresh rate (30-60Hz limited by the depth cameras) and non line-of-sight scenarios. They are also environment-dependent and are not always reliable for any environment and light condition. 


Last but not the least, the mobility nature of AR devices make daily usage of AR devices possible. Users do not prefer bringing so much specific devices with them every time. Hence, we reuse existing devices, most commonly smartphones or smart watches, and realize controller functionality on them. Current controllers for commercial AR devices\cite{magicleap, hololens}, despite do not need base-stations, fail in this perspective as they require bulky dedicated controllers to support high precision tracking.

% propose

Keeping the above challenges in mind, we present \name, an AR gadget that can be easily installed in any existing AR device, to enable real-time sub-millimeter wireless tracking for any smartphone or smart watch. \name use acoustic signal to track a smartphone without any additional base station nor power-consuming sensors such as laser emitter, with a median tracking accuracy of xx mm, yy mm and zz mm for x, y, z dimensions respectively. \name also support up to ll m of operating range which is adequate for handheld interactions. 
To the best of our knowledge, this is the first work that achieve sub-mm accuracy tracking for smartphones without using base-stations.

Specifically, we a) utilize only the existing hardware on off-the-shelf smartphones, which includes computational units, speakers and microphones, and implemented the controller logic totally in software as a library that any app can use; and b) design our gadget prototype for AR glasses which only consists of cheap and low-power electronic components.

The key of achieving such capabilities is a novel signal processing pipeline that, for the first time, achieves 1D acoustic tracking at sub-mm accuracy at XXHz rate with XX ms delay. This not only provides adequate sensitivity, but also eliminates the necessity to use multiple base-stations, as simple angle-of-arrival using the distance differences provides enough angular accuracy using single access-point (\textit{i.e.}, our gadget). 

Specifically, based on our findings from theoretical analysis, we design a filtering algorithm which combines the advantages of chirp localization based on time-of-arrival, and motion tracking based on phase tracking. Theoretically we prove that this improves ~5x accuracy compared to previous work (Section~\ref{sec:theory}, while still maintaining the high sensitivity of phase tracking. This gives us the most accurate one dimensional distance measurement using acoustic signals up to date. Built upon the filtering algorithm is an Angle-of-arrival estimation algorithm to estimate the 3D position of the controller. 

In addition to the acoustic localization scheme, we address some other key challenges to achieve reliable localization. Firstly, we build a simple synchronization algorithm that utilize the symmetric nature of the Doppler effect of the AR glasses and smartphones; Secondly, by making a valid assumption on acceleration (less than $XX m/s^2$), we support arbitrary motion speed which is essential for wireless controllers.  

We implemented our controller prototype on Android platform. For our AR gadget prototype, we use a 3D printer to print the structure of a glasses and stick our sensors into it. The sensors we use are only cheap off-the-shelf speaker \cite{speaker} and microphone \cite{microphones} components. 


% contribution

To summarize, our contributions are:

\begin{itemize}
\item For the first time, we design algorithms to improve the tracking accuracy using acoustic signals into sub-mm territory even in non line-of-sight scenarios.
\item Based on the algorithm, we developed the wireless controller system in two parts, a AR gadget that can be attached in any AR glasses, and an app that can run on any Android smartphones.
\item We perform extensive experiments to verify the usability of our system and evaluate its performance. Experimental results show that our system can achieve a median 3D accuracy of xxx mm with only xxx mm of jitters, within a large working range of xx m. 
\end{itemize}


% The following sections are outlined as follows.

% \begin{itemize}
%     \item Section~\ref{section:challenge} introduces theoretical and practical challenges to build a AR wireless controllers. Physical model and their limitations are also discussed.
%     \item Section~\ref{section:design} elaborates the architecture of our system as well as the detailed design of the algorithms used in our system.
%     \item Section~\ref{section:implementation} describes the design of our software system as well as our hardware prototype.
%     \item Section~\ref{section:evaluation} shows the experimental setup and comprehensive evaluation results of our system in both controlled and free-running experiments.
% \end{itemize}


==> sections/intro_1.tex <==
\section{Introduction}

% Why acoustic localization / tracking

Device localization and motion tracking have long been a key research problem in recent years. They are a vital enabler for Virtual Reality (VR) and Augmented/Mixed Reality (AR), and play a key part in novel human-computer interactions like gesture and skeleton recognition. 
Despite rapid progress in computer vision methods like SLAM\cite{}, they still cannot compete in robustness, accuracy and computational burden.
Recently, acoustic-based localization and tracking methods evolve rapidly\cite{}, and is becoming a potential alternative method to optical methods (laser, IR, etc.) which are widely used in current VR/AR systems.

Acoustic signal above a certain frequency (16-17kHz depending on the age), \textit{i.e.}, ultrasound, is inaudible to human beings. No evidence shows ultrasonic signal in a low sound pressure level harmful to human over an extended period of time\cite{health}. In contrast to RF signals where ISM bands are congested by communication uses\cite{}, consumer speakers and microphones leave around 7kHz empty frequency band for other usages. 
Acoustic signal travels in the speed of sound which is several orders lower than speed of light. As a result, the wavelengths are only a few centimeters long, which makes it more sensitive to motion compared to RF signals. This makes Acoustic signal more suitable for fine-grained motion tracking compared to RF signals.

Acoustic signal can penetrate some occlusions like fabrics. In contrast, laser and IR signals only travel in line-of-sight. 
Moreover, speakers and microphones, used for emitting and receiving acoustic signals, are cheap and easy to configure. Smartphones and smart watches have built-in speaker and microphone, which makes it perfect to adopt acoustic techniques without additional hardware. Current optical tracking solutions, on the other hand, requires separate beacons to emit optical signals. Everyday devices like smartphones are not able to be tracked as well because of lack of optical transceivers.

% What can be enabled

It is natural to ask the following question: Can we enable acoustic localization and tracking in a comparable performance as state-of-the-art optical tracking methods, but without the encumbrance of setting up expensive optical infrastructure? 
A positive answer would allow a much cheaper and more convenient solution to fine-grained localization and motion tracking such as finger tracking and VR/AR headset/controller tracking. Such capability would also benefit everyday devices - smartphones and smart watches, so that we can re-use the existing interface of smartphones and smart watches without the need to buy extra hardware.

% Challenges

However, it is difficult to achieve this because of three major challenges.

\textit{Accuracy}. The most difficult barrier is the accuracy. Over the past few years, a number of acoustic tracking systems have improved the 1D accuracy into 5-10mm range \cite{}, but this is far from the accuracy we can get from optical solutions ($\sim 0.1mm$). The main reason is the law of physics: resolution is lower bounded to $\frac{c}{2B}$ where $c$ is the speed of signal, and $B$ is the bandwidth\cite{}. This translates to around 3cm when we use 6kHz bandwidth. Most objects reflect acoustic signals (echoes) resulting a dense multipath environment. Multiple paths with a distance difference less than 3cm are not separable, resulting biases in the measurement. 
Moreover, the low speed of sound introduce strong Doppler effect when in motion, introducing large bias on the localization measurement.
To combat with this, IMUs are often used to improve the sensitivity\cite{}, but it barely improves the absolute accuracy since IMUs cannot provide absolute measurements. 
Worse, to get acceptable 3D locations using triangulation from multiple 1D measurements, a long separation between multiple speakers or microphones makes them impossible to integrate into VR/AR headsets or most wearables, thus, pre-use stationary beacon setup is still a necessity.

\textit{Agility}. Beside accuracy, a short latency and a high refresh rate is important as well. For example, tracking AR/VR headset with a high latency or a low refresh rate would cause simulator sickness to users\cite{}. It is studied that a latency less than 20ms and a refresh rate higher than 120Hz is preferable for VR/AR applications. However, the low transmission speed and low sampling rate of acoustic signals become a disadvantage: to achieve such agility, receiver should obtain its location using only less than 960 samples (using 48kHz sampling rate).  

\textit{Scalability}. Because of the restricted bandwidth, multiple concurrent transmissions using frequency-division multiplexing (FDM) will reduce the bandwidth per transmission, thus reduce the accuracy. Using time-division multiplexing, on the other hand, trades off the agility.

Despite a number of works over the last few years tried to propose a complete solution, no work is good enough to be able to challenge the existing optical solutions.

% Address the problems

In this paper, we propose \name, a complete acoustic localization system to address all the three challenges. To the best of our knowledge, our work is the first to improve 1D acoustic localization accuracy into sub-mm territory, even in non line-of-sight scenarios, meanwhile only introduce xxms latency and support a refresh rate of xxHz. 

Based on a straightforward mathematical intuition, the core of \name is a novel localization algorithm to achieve real-time sub-mm level 1D localization.
Specifically, the algorithm is designed to combine the advantage of the high agility of phase measurement, and the good multipath rejection capability of linear frequency-modulated continuous wave (FMCW) signals. We dig into math and design our low-complexity algorithm with a proven ~10x accuracy improvement compared to prior work without sacrificing agility.
\name also support up to xx m/s motion speed and up to xx m of operating range which is adequate for room-level interactions.

Moreover, thanks to the high 1D accuracy, we achieve 3D localization of a speaker in a median accuracy of xx mm using four microphones in a separation of as low as 10cm. This makes beacon-less VR/AR controller tracking possible since the 4-microphone array are small enough to fit in a VR/AR headset.

Regarding scalability, our algorithm supports up to xx concurrent transmitters without reducing the accuracy or agility of each transmissions. Because the transmission is one-way except a one-time calibration phase, each transmitter supports tracking unlimited number of receivers. 

% Applications
We envision that our system enables a number of new interaction methods that previously cannot be achieved. Here we list three examples, as illustrated in Fig.~\ref{fig}.

a) AR/VR headset - smart watch tracking. For example, AR/VR Users can draw over the air with only their smart watch worn, and the AR headset precisely captures and shows the masterpieces in real time; They can also play immersive kinetic games tracking their moving arms as precise as a 3D mouse. 

b) Smartphone as a VR/AR beacon. Users can get rid of buying and setting up optical beacons before playing their favorite VR games with their friends - just put your phone on the table, open an App and you are all set. 

c) Accurate finger tracking. Finger rings with cheap speakers can be manufactured in a few dollars. They can be precisely tracked by a nearby smartphone or smart watch. Wearing five of them on each finger, you can play piano over the air with subtle pressure sensing. 

To summarize, our contributions are:

\begin{itemize}
\item For the first time, we design algorithms to improve the 1D tracking accuracy using acoustic signals into sub-mm territory even in non line-of-sight scenarios. 3D location of an median error of xxmm can be inferred by using four microphones with a separation distance of as low as 10cm.
\item Based on the algorithm, we implement our prototype using an Android phone and a customized hardware that can be attached on any VR/AR headsets. 
\item We perform extensive experiments to verify the usability of our system and evaluate its performance. Experimental results show that our system, with only xxms latency, can achieve a median 3D accuracy of xxx mm at xx Hz refresh rate under up to xx m/s motion speed, within a working range of xx m. 
\end{itemize}


==> sections/related_0.tex <==
\section{Related Work}

Related work falls in three categories.

\subsection{Device Localization and Motion Tracking Techniques}

Over the years there emerges various methods to localize and track devices. Those techniques can be grouped into a) Inertial motion tracking; b) Laser, infrared and visible light based localization and tracking; c) radio frequency (RF) localization; and d) acoustic localization and tracking.

\subsubsection{Inertial motion tracking}

Inertial measurement unit (IMU) is one frequently used component to enable motion tracking. IMU senses 3D linear acceleration, rotational rate and heading reference which can be further fused together\cite{fourati2015heterogeneous}. Gaming controllers \cite{switch, wii}, most low-end VR systems\cite{gearvr,oculusgo,daydream} use entirely IMU to support motion tracking.

Using IMU alone however does not support absolute positioning, since it requires double integration of the acceleration, which introduces huge drift error\cite{imuerror}. IMU does improve sensitivity when combined with other methods\cite{mao2016cat}.


\subsubsection{IR and visible light based localization}.
HTC Vive VR\cite{htcvive} system uses a laser beacon named \textit{Lighthouse} emitting coherent IR signal to localize the headset as well as the controllers.
In short, a laser emitter sweep coherent IR light spatially. 3D location can be calculated from the time the IR signals hit the photo-diodes on the receiver and the geometric relationship of the photo-diodes. 

Infrared and visible light from LEDs, albeit not coherent, can be accurately recognized and localized by cameras by using special colors and their geometric relationship. 
Sony PlayStation VR (PSVR)\cite{playstationmove} system use special visible colors to be uniquely recognized and tracked by a standalone camera located in a fixed position. 
Oculus Rift\cite{oculusrift} VR system employs a separate IR camera. The headset and controller are marked with IR LED markers captured by the IR camera. Computer vision algorithms are then applied to obtain the position\cite{rifttracking}.

Despite accurate enough for VR/AR applications, IR and visible light based localization and tracking requires dedicated beacon setup before usage. The working range is limited by the field of view of lasers or IR cameras and the signal cannot penetrate occlusions.
It is also prone to interference from other visible light/IR sources, or when mirrors exist. They also work poorly in bright environments\cite{psvrissue}.

\subsubsection{RF localization and tracking}

Radio Frequency (RF) signal can be used for localization and tracking.
Cricket\cite{cricket} utilize the speed difference of RF signal and acoustic signal to achieve a median 3D error of 12cm. ArrayTrack\cite{arraytrack} use a 16-antenna array to achieve a median 3D error of 23cm using WiFi. SpotFi\cite{spotfi} achieve WiFi localization accuracy to 40cm using an off-the-shelf access point. WiCapture\cite{wicapture} improves the median tracking accuracy to 0.88cm but requires multiple distanced APs as beacons. \cite{ma2017minding} achieves 0.91cm median RFID tag localization accuracy using a large bandwidth that exceeds ISM bands.
% MTrack\cite{wei2015mtrack} uses 60GHz millimeter wave to achieve 6mm median error but requires expensive 60GHz infrastructure.

Because of the relatively small available bandwidth and fast transmission speed, the accuracy of RF localization is not suitable for fine-grained tracking.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
System                & Setup                                                                        & \begin{tabular}[c]{@{}l@{}}Ranging\\ technique\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}Need\\ IMU\end{tabular} & Audible            & Dimension & Accuracy & Latency               & \begin{tabular}[c]{@{}l@{}}Refresh\\ rate\end{tabular} & Range               & \begin{tabular}[c]{@{}l@{}}Concurrent\\ transmission\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Mic/speaker\\ Separation\end{tabular}          \\ \hline
BeepBeep              & Phone-Phone                                                                  & Autocorrelation                                                                 & N                                                  & Y                  & 1D        & 2cm      & 50ms                  & 20Hz                                                   & 12m                    & N                                             & -                                                                            \\ 
Swordfight            & Phone-Phone                                                                  & Autocorrelation                                                                 & N                                                  & Y                  & 1D        & 2cm      & 46ms                  & 12Hz                                                   & 3m                   & N                                                 & -                                                                             \\ 
BatTracker            & \begin{tabular}[c]{@{}l@{}}Phone self-\\ localization\end{tabular}            & \begin{tabular}[c]{@{}l@{}}Autocorrelation+\\ Particle filter\end{tabular}      & Y                                                  & N                  & 3D        & 5mm      & -                     & 32Hz                                                   & 3m                   & N                                                 & -                                                                            \\
CAT                   & Speaker-Phone                                                                & FMCW                                                                            & Y                                                  & N                  & 3D        & 9mm      & 40ms                  & 25Hz                                                   & 7m                   & N                                               & 90cm                                                                          \\ 
SoundTrak             & Speaker-Watch                                                                & Phase tracking                                                                  & N                                                  & Y                  & 3D        & 13mm     & 12ms                  & 86Hz                                                   & 20cm                 & N                                               & 4cm                                                                           \\ 
Sonoloc               & Phone-Phone                                                                  & Autocorrelation                                                                 & N                                                  & Y                  & 2D        & 6cm      & 3.2-48s               & -                                                      & 17m                  & N                                                 & -                                                                             \\ \hline
\multirow{2}{*}{\name} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Microphone-\\ Phone\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}FMCW+\\ Phase tracking\end{tabular}} & \multirow{2}{*}{N}                                 & \multirow{2}{*}{N} & 3D        & 1.5mm    & \multirow{2}{*}{15ms} & \multirow{2}{*}{\textgreater{}66Hz}                    & \multirow{2}{*}{3m} & \multirow{2}{*}{Y}                               & \multirow{2}{*}{10cm}                                        \\ \cline{6-7}
                      &                                                                              &                                                                                 &                                                    &                    & 1D        & 0.6mm    &                       &                                                        &                                        &                                 &                                                                                   \\ \hline
\end{tabular}
}
\end{table*}

\subsubsection{Acoustic localization and tracking}

Our work falls into this category. We list recent works on acoustic localization and tracking in Table~\ref{tab:acousticworks}. Specifically, BeepBeep\cite{beepbeep} and Swordfight\cite{zhang2012swordfight} track 1D distances between phones but not 3D locations. Despite no beacon needed, BatTracker\cite{battracker} requires computational-extensive particle filter. Sonoloc\cite{sonoloc} realizes distributed localization and requires 10+ devices to achieve reasonable accuracies. 
CAT\cite{mao2016cat} and SoundTrak\cite{zhang2017soundtrak} are most comparable to our work. CAT achieves a median 3D error of 9mm using a combination of IMU sensor data and FMCW localization. It requires a separation of 0.9m and 0.7m between its horizontal and vertical speaker pairs respectively. SoundTrak\cite{zhang2017soundtrak} achieves an average 3D error of 1.3cm between a smart watch and a customized finger ring using phase tracking but the area of movement is limited to a $20cm\times16cm\times11cm$ space.

Compared with all those works, \name achieves a much higher accuracy and good agility, because of our novel tracking algorithms for FMCW signals, .


\subsection{Simultaneous Localization and Mapping (SLAM)}

Unlike previous methods, SLAM is an inside-out tracking method, which means that it does not rely on any infrastructure and locate the device itself solely based on the environment captured by its camera.
AR systems such as Microsoft Hololens\cite{hololens} and Magic Leap One\cite{magicleap} headset use SLAM to locate themselves meanwhile reconstruct the surrounding environment to support augmented reality.
SLAM performance highly depends on the environment such as light condition and variety of visual features. Hence, it is not as robust as outside-in tracking methods. SLAM is also a computational intensive algorithm that often requires specialized hardware accelerator to support real-time tracking. Because of this, SLAM is not appropriate for tracking tiny controllers.


\subsection{Device-free Interactions}

Kinect\cite{kinect} use IR cameras to recognize human skeleton without any wearable devices. Leap Motion\cite{leapmotion} and Google Soli\cite{googlesoli} recognize hand motion using millimeter wave and IR signal respectively. They requires additional hardware and cannot track the accurate position. FingerIO\cite{fingerio} and LLAP\cite{llap} use acoustic signals to recognize finger motion in sub-centimeter accuracy, but the range is limited because they rely on the reflection on the fingers. ApneaApp\cite{apnea} use acoustic signals to monitor breath and Apnea event but it cannot track arbitrary motion. StarLight\cite{li2016practical} realizes skeleton tracking using visible light which requires LED infrastructure setup on the ceiling.

A number of works take advantages of machine learning to classify different motions using wireless signals \cite{zhao2018rf, wisee, gupta2012soundwave,laput2015acoustruments, zhang2017fingersound}, but they requires training data before inference task. 


==> sections/theory_0.tex <==
\section{Towards sub-mm level acoustic tracking}

In this section, we theoretically analyze the accuracy of different tracking methods. Our key finding  
